LANA: Latency Aware Network Acceleration

We introduce latency-aware network acceleration (LANA) - an approach that builds on neural architecture search techniques and teacher-student distillation to accelerate neural networks. LANA consists of two phases: in the first phase, it trains many alternative operations for every layer of the teacher network using layer-wise feature map distillation. In the second phase, it solves the combinatorial selection of efficient operations using a novel constrained integer linear optimization (ILP) approach. ILP brings unique properties as it (i) performs NAS within a few seconds to minutes, (ii) easily satisfies budget constraints, (iii) works on the layer-granularity, (iv) supports a huge search space $O(10^{100})$, surpassing prior search approaches in efficacy and efficiency. In extensive experiments, we show that LANA yields efficient and accurate models constrained by a target latency budget, while being significantly faster than other techniques. We analyze three popular network architectures: EfficientNetV1, EfficientNetV2 and ResNeST, and achieve accuracy improvement for all models (up to $3.0\%$) when compressing larger models to the latency level of smaller models. LANA achieves significant speed-ups (up to $5\times$) with minor to no accuracy drop on GPU and CPU. The code will be shared soon.

==> LANA_CVPR2022_arxiv%20(Version%20281)/0_abstract.tex <==
\begin{abstract}
We introduce latency-aware network acceleration (LANA) – an approach that builds on neural architecture search techniques and teacher-student distillation to accelerate neural networks. LANA consists of two phases: in the first phase, it trains many alternative operations for every layer of the teacher network using layer-wise feature map distillation. In the second phase, it solves the combinatorial selection of efficient operations using a novel constrained integer linear optimization (ILP) approach. ILP brings unique properties as it (i) performs NAS within a few seconds to minutes, (ii) easily satisfies budget constraints, (iii) works on the layer-granularity, (iv) supports a huge search space $O(10^{100})$, surpassing prior search approaches in efficacy and efficiency.

In extensive experiments, we show that LANA yields efficient and accurate models constrained by a target latency budget, while being significantly faster than other techniques. We analyze three popular network architectures: EfficientNetV1, EfficientNetV2 and ResNeST, and achieve up to $3.0\%$ accuracy improvement for all models when compressing larger models to the latency level of smaller models. LANA achieves significant speed-ups (up to 5$\times$) with minor to no accuracy drop on GPU and CPU. The code will be available soon.
\end{abstract}



==> LANA_CVPR2022_arxiv%20(Version%20281)/0_introduction.tex <==
\vspace{-0.5cm}
\section{Introduction}
\label{sec:intro}
In many applications, we may have access to a neural network that satisfies desired performance needs in terms of accuracy but is computationally too expensive to deploy. The goal of hardware-aware network acceleration~\cite{rastegari2016xnor, zhang1707shufflenet, sze2017efficient, he2018amc, cai2020once, chamnet} is to accelerate a given neural network such that it meets efficiency criteria on a device without sacrificing accuracy dramatically. Network acceleration plays a key role in reducing the operational cost, power usage, and environmental impact of deploying deep neural networks in real-world applications. 


The current network acceleration techniques can be grouped into: \textit{(i) pruning} that removes inactive neurons~\citep{mozer1989skeletonization, lecun1990optimal, hanson1989comparing, chauvin1989back, molchanov2016pruning, molchanov2019importance, thinet, liu2018rethinking, nisp, he2018soft, he2019filter, frankle2018lottery, he2017channel, zhu2016trained, lebedev2016fast,li2016pruning, ICLR2018, he2018adc, louizos2017learning, neklyudov2017structured, he2016identity,huang2017densely, gordon2018morphnet, yu2017nisp, he2018progressive, molchanov2017variational, blalock2020state}, (ii) \textit{compile-time optimization}~\cite{Ryoo2008OptimizationPA} \textit{or kernel fusion}~\citep{Wang2010KernelFA, ding2021repvgg, ding2019acnet, zagoruyko2017diracnets} that combines multiple operations into an equivalent operation, (iii) \textit{quantization} that reduces the precision in which the network operates at~\citep{wang2019haq, dong2019hawq, shen2020qbert, cai2020zeroq, Choi2018PACTPC, Park2018ValueawareQF, Wu2018MixedPQ, Zhang2018LQNetsLQ, Krishnamoorthi2018QuantizingDC}, and \textit{(iv) knowledge distillation} that distills knowledge from a larger \textit{teacher} network into a smaller \textit{student} network~\citep{hinton2015distilling, sau2016deep, xu2017training,yin2020dreaming,mishra2017apprentice, nayak2019zero, belagiannis2018adversarial}. The approaches within (i) to (iii) are restricted to the underlying network operations and they do not change the architecture. Knowledge distillation changes the network architecture from teacher to student, however, the student design requires domain knowledge and is done usually manually. 

\input{tables/method_comparison}

In this paper, we propose latency-aware network transformation (LANA), a network acceleration framework that automatically replaces inefficient operations in a given network with more efficient counterparts. Given a convolutional teacher network, we formulate the problem as searching in a large pool of candidate operations to find efficient operations for different layers of the teacher. The search problem is combinatorial in nature with a space that grows exponentially with the depth of the network. To solve this problem, we can turn to neural architecture search (NAS)~\citep{zoph2016neural, zoph2018learning, tan2018mnasnet, cai2018proxylessnas, pham2018efficient, vahdat2020unas}, which has been proven successful in discovering novel architectures. However, existing NAS solutions are computationally expensive, and usually handle only a small number of candidate operations (ranging from 5 to 15) in each layer and they often struggle with larger candidate pools.

To tackle the search problem with a large number of candidate operations in an efficient and scalable way, we propose a two-phase approach. In the first phase, we define a large candidate pool of operations ranging from classic residual blocks \citep{he2016deep} to recent blocks~\citet{dosovitskiy2020image, ding2021repvgg, srinivas2021bottleneck, bello2021lambdanetworks}, with varying hyperparameters. 
Candidate operations are pretrained to mimic the teacher's operations via a simple layer-wise optimization.
Distillation-based pretraining enables a very quick preparation of all candidate operations, offering a much more competitive starting point for subsequent searching.

In the second phase, we search among the pre-trained operations as well as the teacher's own operations to construct an efficient network. Since our operation selection problem can be considered as searching in the proximity of the teacher network in the architecture space, we assume that the accuracy of a candidate architecture can be approximated by the teacher's accuracy and a simple linear function that measures changes in the accuracy for individual operations. Our approximation allows us to relax the search problem into a constrained integer linear optimization problem that is solved in a few seconds. As we show extensively in our experiments, such relaxation can drastically cut down on the cost of our search and it can be easily applied to a huge pool of operations (197 operations per layer), while offering improvements in model acceleration by a large margin. 

In summary, we make the following contributions: \textbf{(i)} We propose a simple two-phase approach for accelerating a teacher network using NAS-like search. \textbf{(ii)} We propose an effective search algorithm using constrained integer optimization that can find an architecture in seconds tailored to our setting where a fitness measure is available for each operation. \textbf{(iii)} We examine a large pool of operations including the recent vision transformers and new variants of convolutional networks. We provide insights into the operations selected by our framework and into final model architectures. 



\vspace{-0.0cm}
\subsection{Related Work}

Since our goal is to discover new efficient architectures, in this section we focus on related NAS-based approaches.  

\textbf{Hardware-aware NAS:} The goal of hardware-aware NAS is to %When looking to automatically identifying architectures to maximize both accuracy and computational efficiency, there are two main lines of work. One is to 
design efficient and accurate architectures from scratch while targeting a specific hardware platform. This has been the focus of an increasingly large body of work on multiobjective neural architecture search \citep{cai2018proxylessnas, Tan_2019_CVPR, Wu_2019_CVPR, yang2018netadapt, veniat2017learning, yang2018synetgy, wu2018mixed, vahdat2020unas}. The goal here is to solve an optimization problem maximizing accuracy while meeting performance constraints specified in terms of latency, memory consumption or number of parameters. Given that the optimization problem is set up from scratch for each target hardware platform, these approaches generally require the search to start from scratch for every new deployment target (\emph{e.g.}, GPU/CPU family) or objective, incurring a search cost that increases linearly as the number of constraints and targets increases. \citet{cai2020once} circumvents this issue by training a supernetwork containing every possible architecture in the search space, and then applying a progressive shrinking algorithm to produce multiple high-performing architectures. This approach incurs a high pretraining cost, but once training is complete, new architectures are relatively inexpensive to find. On the other hand, the high computational complexity of pretraining limits the number of operations that can be considered. Adding new operations is also costly, since the supernetwork must be pretrained from scratch every time a new operation is added. % And because of the progressive shrinking search algorithm, only a restricted set of operations are supported by this approach.

\textbf{Teacher-based NAS:} Our work is more related to the line of work that focuses on modifying \emph{existing} architectures. Approaches in this area build on teacher-student knowledge distillation, performing multiobjective NAS on the student to mimic the teacher network. Pioneering works \cite{Liu_2020_CVPR}, \cite{Li_2020_CVPR} and \cite{moons2020distilling} demonstrated great benefits of teacher-student NAS, however, can be improved.

The AKD approach \cite{Liu_2020_CVPR} applies knowledge distillation at the network level, training a reinforcement learning agent to construct an efficient student network given a teacher network and a constraint and then training that student from scratch using knowledge distillation. DNA~\citet{Li_2020_CVPR} and DONNA~\citet{moons2020distilling} take a more fine-grained approach, dividing the network into a small number of blocks, each of which contain several layers. 
During knowledge distillation, they both attempt to have student blocks mimic the output of teacher blocks, but \cite{Li_2020_CVPR} samples random paths through a mix of operators in each block, whereas \citet{moons2020distilling} trains several candidate blocks with a repeated single operation for each teacher block. They then both search for an optimal set of blocks, with DNA~ \citet{Li_2020_CVPR} using a novel ranking algorithm to predict the best set of operations within each block, and then applying a traversal search, 
while \citet{moons2020distilling} train a linear model that predicts accuracy of a set of blocks and use that to guide an evolutionary search. While both methods deliver impressive results, they differ from our approach in important ways. DNA~\citet{Li_2020_CVPR} ranks each path within a block, and then use this ranking to search over the blocks, relying on the low number of blocks to accelerate search. DONNA \citet{moons2020distilling} samples and finetunes 30 models to build a linear accuracy predictor, which incurs a significant startup cost for search. In contrast, we formulate the search problem as an integer linear optimization problems that can be solved very quickly for large networks and large pool of operations.

Table~\ref{tab:related_work} compares our work to these works in detail. We increase the granularity of network acceleration, focusing on each \emph{layer} individually instead of blocks as done in DNA and DONNA. The main advantage of focusing on layers is that it allows us to accelerate the teacher by simply \textit{replacing} inefficient layers whereas blockwise algorithms such as DNA and DONNA require \textit{searching} for an efficient subnetwork that mimics the whole block. The blockwise search introduces additional constraints. For example, both DNA and DONNA enumerate over different depth values (multiplying the search space) while we reduce depth simply using an identity operation. Additionally, DONNA assumes that the same layer in each block is repeated whereas we have more expressivity by assigning different operation to different layers.  The expressivity can be seen from the design space size in Table~\ref{tab:related_work} in which our search space is orders of magnitude larger.
On the other hand, this extremely large space necessitate the development of a highly efficient search method based on integer linear optimization (presented in Section~\ref{sec:method}). As we can see from Table~\ref{tab:related_work}, even with significantly larger search space, our total cost is lower than prior work. We additionally introduce zero-shot formation when the teacher cell and the identity operations participate in ILP, reducing the pretraining and the search costs to a minimum.

==> LANA_CVPR2022_arxiv%20(Version%20281)/0_metadata.tex <==
\title{LANA: Latency Aware Network Acceleration}

\author{TBD\\
NVIDIA\\
{\tt\small dannyy@nvidia.com}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
}




% \title{[CVPR2022] Official LaTeX Template}

% \author{Andrea Tagliasacchi\\
% Google Research \& University of Toronto\\
% {\tt\small taglia@google.com}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% % \and
% % Second Author\\
% % Institution2\\
% % First line of institution2 address\\
% % {\tt\small secondauthor@i2.org}
% }

==> LANA_CVPR2022_arxiv%20(Version%20281)/1_method.tex <==
\section{Method}
\label{sec:method}


\begin{figure*}[ht!]
\vspace{-0.0cm}\centering
\begin{subfigure}[t]{.4\textwidth}
\includegraphics[width=1.\textwidth]{images/Distillation.pdf}
\caption{\textbf{Candidate pretraining phase:} We minimize the MSE loss between the output of the teacher operation \(t_{i}\) and the output of each student operation on each layer \(s_{i,j}\), where the input to each operation is the teacher output from the previous layer.}
\end{subfigure}
\hspace{1mm}
\unskip\ \vrule\
\hspace{1mm}
\begin{subfigure}[t]{.4\textwidth}
\includegraphics[width=0.95\textwidth]{images/SelectDistill.pdf}
\caption{\textbf{Operation Selection Phase:} We estimate and record in a lookup table the reduction of network accuracy and latency from replacing a teacher operation with one of the student operations. We then apply integer programming to minimize the accuracy reduction while attaining a target latency reduction.}
\end{subfigure}
\vspace{0.5cm}
\caption{\small LANA consists of two phases: a candidate pretraining phase (a) and an architecture search phase (b).\label{fig:method}}
\end{figure*}

Our goal in this paper is to accelerate a given pre-trained teacher network by replacing its inefficient operations with more efficient alternatives. Our method, visualized in Fig.~\ref{fig:method}, is composed of two phases: (i) \emph{Candidate pretraining phase} (Sec.~\ref{sec:pretraining}), in which we use distillation to train a large set of operations to approximate different layers in the original teacher architecture; (ii) \emph{Operation selection phase} (Sec.~\ref{sec:search}), in which we search for an architecture composed of a combination of the original teacher layers and pretrained efficient operations via linear optimization.

\subsection{Candidate Pretraining Phase} \label{sec:pretraining}


%\textbf{Notation:} 
We represent the teacher network as the composition of $N$ teacher operations by \(\mathcal{T}\left(x\right) = t_{N} \circ t_{N - 1 } \circ \ldots \circ t_{1} \left(x\right)\), where $x$ is the input tensor, $t_{i}$ is the $i^\textrm{th}$ operation (i.e., layer) in the network.
We then define the set of \emph{candidate student operations} \(\bigcup_{i=1}^{N}\left\{s_{ij}\right\}_{j=1}^{M}\), which will be used to approximate the teacher operations. Here, $M$ denotes the number of candidate operations per layer. The student operations can draw from a wide variety of operations
-- the only requirement is that all candidate operations for a given layer must have the same input and output tensor dimensions as the teacher operation \(t_{i}\). 
We denote all the parameters (e.g., trainable convolutional filters) of the operations as $\mathbf{W} = \{w_{ij}\}_{i,j}^{N,M}$, where $w_{ij}$ denotes the parameters of the student operation $s_{ij}$. We use a set of binary vectors $\mathbf{Z} = \left\{\mathbf{z}_i\right\}_{i=1}^{N}$, where $\mathbf{z}_{i}=\{0, 1\}^M$ is a one-hot vector, to represent operation selection parameters. We denote the candidate network architecture specified by $\mathbf{Z}$ using $\mathcal{S}(x; \mathbf{Z}, \mathbf{W})$. % with operation weights $\mathbf{W}$. 

The problem of optimal selection of operations is often tackled in NAS. This problem is usually formulated as a bi-level optimization that selects operations and optimizes their weights jointly \citep{liu2018darts, zoph2016neural}.
Finding the optimal architecture in hardware-aware NAS reduces to: % solving the following joint combinatorial integer optimization problem and weight training:
\begin{align}
   \min_{\mathbf{Z}} \min_{\mathbf{W}} \quad & \underset{\textrm{objective}}{ \sum_{(x, y) \in X_{tr}}\mathcal{L}\big(\mathcal{S}(x; \mathbf{Z}, \mathbf{W}), y\big)}, &\label{eq:nas_formulation} \\
\textrm{s.t.} \quad & \underset{\textrm{budget constraint}}{\sum_{i=1}^N \mathbf{b}_{i}^T \mathbf{z}_i \leq \mathcal{B}}\ ; %\\
 \quad  \underset{\textrm{one op per layer}}{\mathbf{1}^T \mathbf{z}_i = 1\ \forall\ i\in[1..N]} \nonumber
\end{align}
where $\mathbf{b}_{i} \in \mathbb{R}_+^M$ is a vector of corresponding cost of each student operation (latency, number of parameters, FLOPs, etc.) in layer~\(i\). The total budget constraint is defined via scalar $\mathcal{B}$. The objective is to minimize the loss function $\mathcal{L}$ that estimates the error with respect to the correct output $y$ while meeting a budget constraint. 
In general, the optimization problem in Eq.~\ref{eq:nas_formulation} is an NP-hard combinatorial problem with an exponentially large state space (i.e., $M^N$). 
The existing NAS approaches often solve this optimization using evolutionary search~\citep{real2017large}, reinforcement learning~\citep{zoph2016neural} or differentiable search~\citep{liu2018darts}. 

However, the goal of NAS is to find an architecture in the whole search space from scratch, whereas our goal is to improve efficiency of a given teacher network by replacing operations. Thus, our search can be considered as searching in the architecture space in the proximity of the teacher network. That is why we assume that the functionality of each candidate operation is also similar to the teacher's operation, and we train each candidate operation to mimic the teacher operation 

using layer-wise feature map distillation with the mean squared error (MSE) loss:
\begin{equation} \label{eq:mse}
    \min_{\mathbf{W}} \sum_{x \in X_\textrm{tr}} \sum_{i,j}^{N,M}  \left\| t_{i}(x_{i-1}) - s_{ij}(x_{i-1}; w_{ij}) \right\|_2^2,
\end{equation}
where $X_\textrm{tr}$ is a set of training samples, and $x_{i-1}=t_{i-1}\circ t_{i-2}\circ \ldots \circ t_\text{1}\left(x\right)$ is the output of the previous layer of the teacher, fed to both the teacher and student operations. 

Our layer-wise pretraining has several advantages. First, the minimization in Eq.~\ref{eq:mse} can be decomposed into $N \times M$ independent minimization problems as $w_{i,j}$ is specific to one minimization problem per operation and layer. This allows us to train all candidate operations simultaneously in parallel. Second, since each candidate operation is tasked with an easy problem of approximating \textit{one} layer in the teacher network, we can train the student operation quickly in one epoch. In this paper, instead of solving all $N \times M$ problems in separate processes, we train a single operation for each layer in the same forward pass of the teacher to maximize reusing the output features produced in all the teacher layers. This way the pretraining phase roughly takes \(O(M)\) epochs of training a full network. 

\iffalse
For both operation pretraining and architecture finetuning, we use a generic knowledge distillation loss function. Given a teacher architecture \(\mathcal{T}\) and a student architecture \(\mathcal{S}\), we define this as the loss approximating the student loss function and its proximity to the teacher on an input-label pair \(\left(x, y\right)\):
%

{\vspace{-0.0cm} \small
\begin{align}
    \mathcal{L}_{\text{dist}}\left({\mathcal{T}}, \mathcal{S}, x, y\right) =\gamma_{\text{MSE}}\sum_i^N  \left\|{s}_{i}(x_{i-1}) - t_{i}(x_{i-1})\right\|_{2}^2 + \gamma_\textrm{CE}  \mathcal{L}_\textrm{CE}\left(\mathcal{S}(x), y\right)
    + \gamma_\textrm{KL}  \mathcal{L}_\textrm{KL}\left(\mathcal{T}(x), \mathcal{S}(x)\right),
    \label{eq:main_loss}
    %+ \gamma_{KL} \left\| \mathcal{F} - \tilde{\mathcal{F}_{i j}}\right\|_{KL}
\end{align} \vspace{-0.0cm}
}

%
where the first term is the mean squared error (MSE) loss, $\mathcal{L}_\textrm{CE}(\cdot)$ is a cross entropy loss,  $\mathcal{L}_\textrm{KL}(\cdot)$ is a Kullback–Leibler (KL) divergence; $\gamma_{\textrm{MSE}}$, $\gamma_{\textrm{CE}}$ and $\gamma_{\textrm{KL}}$ are corresponding scaling coefficients; $x_{i-1}=t_{i-1}\circ t_{i-2}\circ \ldots \circ t_\text{in}\left(x\right)$ is the output of the previous layer of the teacher, so that the teacher and student operations are applied to the same input. 

Denote the weights for the student operation \(s_{ij}\) as \(w_{ij}\). For pretraining, our goal is to find a set of weights $\mathcal{W} = \bigcup_{i=1}^{N}\{w_{ij}\}_{j=1}^{M}$ that minimizes the distillation loss over all architectures and over all pairs \(\left\{\left(x, y\right)\right\} = X_{tr}\) in our training set (which together we call the \emph{pretraining loss}, \(\mathcal{L}_{\textrm{pt}}\)), i.e., \(\min_{\mathcal{W}}\mathcal{L}_{\textrm{pt}}\left(X_\textrm{tr}, \mathcal{T}, \mathfrak{S}\right)\), where \(\mathfrak{S}\) is the set of all student networks and  \(\mathcal{L}_{\textrm{pt}}\left(X_\textrm{tr}, \mathcal{T}, \mathfrak{S}\right) = \sum_{\left(x, y\right) \in X_\textrm{tr}} \sum_{\mathcal{S} \in \mathfrak{S}} \mathcal{L}_{\textrm{dist}} \left(\mathcal{T}, \mathcal{S}, x, y\right)\).


To make pretraining efficient, we set \(\gamma_{\textrm{CE}} = 0\) and \(\gamma_{\mathrm{KL}} = 0\). The minimization of the loss function \(\mathcal{L}_{\textrm{pt}}\) becomes (dropping the intermediate feature map $x_j$ for the ease of notation):
%
\begin{align}
    \min_{\mathcal{W}}\mathcal{L}_{\textrm{pt}}\left(X_\textrm{tr}, \mathcal{T}, \mathfrak{S}\right) = \min_{\mathcal{W}} \big(\sum_{\left(x,y\right)} \sum_{\mathcal{S} \in \mathfrak{S}} \gamma_{\textrm{MSE}}\sum_i^N  \left\|t_{i} - s_{i}\right\|_{2}^2\big) = \sum_{\left(x, y\right)} \sum_{i,j}^{N,M} \min_{w_{ij}} \left\| t_{j} - s_{ij} \right\|_2^2,

    \label{eq:mse}
\end{align}
%
where on the right hand side minimization is done on individual candidate operation $s_{ij}$, since \(\left\|t_{j} - s_{ij}\right\|\) does not depend on \(w_{nm}\) if \(nm \neq ij\). In other words, we can minimize the objective by minimizing the expected MSE loss between each candidate operation and the teacher operation for its layer. % 
%
\fi

\subsection{Operation Selection Phase} \label{sec:search}
Since our goal in search is to discover an efficient network in the proximity of the teacher network, we propose a simple linear relaxation of candidate architecture loss using 
\begin{equation}
    \sum_{ X_{tr}}\mathcal{L}\big(\mathcal{S}(x; \mathbf{Z}), y\big) \approx \sum_{X_{tr}}\mathcal{L}\big(\mathcal{T}(x), y\big) + \sum_{i=1}^N \mathbf{a}_{i}^T \mathbf{z}_i,
\end{equation}
where the first term denotes the training loss of teacher which is constant and $\mathbf{a}_{i}$ is a vector of change values in the training loss per operation for layer \(i\). Our approximation bears similarity to the first-degree Taylor expansion of the student loss with the teacher as the reference point (since the teacher architecture is a member of the search space). To compute $\{\mathbf{a}_{i}\}_{i}^N$, after pretraining operations in the first stage, we plug each candidate operation one-by-one in the teacher network and we measure the change on training loss on a small labeled set. Our approximation relaxes the non-linear loss to a linear function. Although this is a weak approximation that ignores how different layers influence the final loss together, we empirically observe that it performs well in practice as a proxy for searching the student. 

\iffalse
computed over a small search set \(X_\textrm{se}\).
\textbf{Linear relaxation: }
The availability of the teacher network allows us to measure the fitness of each operation when it is plugged individually one-by-one in the teacher network. We call this metric as an operation's score. This way, we can measure how much each candidate operation at each layer changes teacher's overall loss $\mathcal{L}$ on a small labeled set. 
Given this, we propose to relax the optimization problem in Eq.~\ref{eq:nas_formulation} to an integer linear problem in which the complex loss function $\mathcal{L}$ is replaced with a linear combination of losses (or equally changes in losses) per operation after the pretraining. This proxy relaxes the non-linear objective to a linear problem. Although, this is a weak approximation that assumes independence of the input to \(i^{\textrm{th}}\) operations from the choice of operations at layers up to \(i-1\), we empirically observe that it performs well in practice when searching in the candidate architecture space. 
\fi

Approximating the architecture loss with a linear function allows us to formulate the search problem as solving an integer linear program (ILP). This has several main advantages: (i) Although solving integer linear programs is generally NP-hard, there exist many off-the-shelf libraries that can obtain a high-quality solutions in a few seconds.  (ii) Since integer linear optimization libraries easily scale up to millions of variables, our search also scales up easily to very large number of candidate operations per layer.  (iii) We can easily formulate the search problem such that instead of one architecture, we obtain a set of diverse candidate architectures.
Formally, we denote the $k^\text{th}$ solution with \(\left\{\mathbf{Z}^{\left(k\right)}\right\}_{k=1}^{K}\), which is obtained by solving:
%
\begin{align}      
\min_{\textbf{Z}^{(k)}} \underset{\textrm{objective}}{\sum_{i=1}^N \mathbf{a}_{i}^T \mathbf{z}^{(k)}_i}, \
 \textrm{s.t.} & \ \underset{\textrm{budget constraint}}{\sum_{i=1}^N \mathbf{b}_{i}^T \mathbf{z}_{i}^{\left(k\right)}\leq \mathcal{B}};
\ \underset{\textrm{one op per layer}}{\mathbf{1}^T \mathbf{z}_{i}^{\left(k\right)} = 1\ \forall\ i}; \nonumber \\
& \ \underset{\textrm{overlap constraint}}{\sum_{i=1}^N {\mathbf{z}_{i}^{(k)}}^{T} \mathbf{z}^{(k')}_i} \leq \mathcal{O}, \forall k' < k  \label{eq:integer} 
\end{align}
% $\mathbf{a}_{i}$ is a vector of proxy expected loss per operation for layer \(i\). %, computed over a small search set \(X_\textrm{se}\). 
where we minimize the change in the loss while satisfying the budget and overlap constraint.
The scalar $\mathcal{O}$ sets the maximum overlap with any previous solution which is set to \(0.7N\) in our case. We obtain $K$ diverse solutions by solving the minimization above $K$ times.

\textbf{Solving the integer linear program (ILP).} % While solving Eq.~\ref{eq:integer} is still NP-hard, the problem of linear integer programming has been well studied and there exist many good approximate solution techniques. For example, i) enumeration techniques (including the branch-and-bound procedure); ii) cutting-plane techniques; and iii) group-theoretic techniques are all effective for approximating the solution of the optimization problem. We refer the reader to the general description of solvers in~\cite{optimization_mit}. 
We use the off-the-shelf PuLP Python package to find feasible candidate solutions. % \(\left\{\mathbf{Z}^{\left(k\right)}\right\}_{k=1}^{K}\) by using all available solvers for each \(k\) and selecting the best candidate (lowest approximate loss) from these solutions. 
The cost of finding the first solution is very small, often less than 1 CPU-second. As \(K\) increases, so does the difficulty of finding a feasible solution. We limit \(K\) to $\sim$100.

\textbf{Candidate architecture evaluation.} Solving Eq.~\ref{eq:integer} provides us with $K$ architectures. The linear proxy used for candidates loss is calculated in an isolated setting for each operation. To reduce the approximation error, we evaluate all $K$ architectures with pretrained weights from phase one on a small part of the training set (6k images on ImageNet) and select the architecture with the lowest loss. % Batch normalization layers have to be open and use current batch statistics to adopted for changed operations. 

\textbf{Candidate architecture fine-tuning.} After selecting the best architecture among the $K$ candidate architectures, we fine-tune it for 100 epochs using the original objective used for training the teacher. Additionally, we add the distillation loss from teacher to student during fine-tuning. %The number of training epochs is reduced to 100. 


==> LANA_CVPR2022_arxiv%20(Version%20281)/2_2_analysis.tex <==
\subsection{Analysis}

% LANA relies on multiple concepts such as linear relaxation, candidate operations scoring, integer linear programming (ILP). 
% Here, we study these concepts in detail using EfficientNetV2-B3 as the teacher for most ablations.

Here, we provide detailed ablations to analyze our design choices in LANA for both pretraining and search phases, along with observed insights. Unless otherwise stated, we used EfficientNetV2-B3 as our teacher for the ablation.

\textbf{Linear relaxation} in architecture search assumes that a candidate architecture can be scored by a fitness metric measured independently for all operations. 
Although this relaxation is not accurate, we observe a strong correlation between our linear objective and the training loss of the full architecture.
This assumption is verified by sampling 1000 architectures (different budget constraints), optimizing the ILP objective, and measuring the real loss function. Results are shown in Fig.~\ref{fig:ILP_analysis}\subref{fig:linear_relaxation} using the train accuracy as the loss. We observe that ILP objective ranks models with respect to the measured accuracy correctly under different latency budgets. The Kendall Tau correlation is $0.966$.


To evaluate the quality of the solution provided with ILP, we compare it with random sampling. The comparison is shown in Fig.~\ref{fig:ILP_analysis}\subref{fig:ilp_vs_random}, where we sample 1000 random architectures for 7 latency budgets. The box plots indicate the poor performance of the randomly sampled architectures. 
The first ILP solution has significantly higher accuracy than random architecture. Furthermore, finding multiple diverse solutions is possible with ILP using the overlap constraint. If we increase the number of solutions found by ILP from $K{=}1$ to $K{=}100$, performance improves further. 


\begin{figure*}
     \centering
         \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=1.\textwidth,trim={0 0 0px 0},clip]{images/v2/integer_optimization_efnv2_b3_latency_False.pdf}
         \caption{Optimization objective}
         \label{fig:linear_relaxation}
     \end{subfigure}\hspace{5mm}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=1.\textwidth,trim={0 0cm 0px 0},clip]{images/v2/ilp_nas.pdf}
         \caption{ILP vs random}
         \label{fig:ilp_vs_random}
     \end{subfigure}\hspace{5mm}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=1.\textwidth,trim={0 0 0px 0},clip]{images/v2/test_accuracy_correlation_vs_train.pdf}
         \caption{Candidate evaluation}
         \label{fig:candidate_evaluation}
     \end{subfigure}
     \vspace{6mm}
        \caption{Analyzing ILP performance on EfficientNetV2-B3. ILP results in significantly higher model accuracy before finetuning than 1k randomly sampled architectures in (\subref{fig:ilp_vs_random}). Accuracy monotonically increases with ILP objective (\subref{fig:linear_relaxation}). Model accuracy before finetuning correctly ranks models after finetuning (\subref{fig:candidate_evaluation}). Train top-1 is measured \textit{before} finetuning, while Validation top-1 is \textit{after}.
        }
        
        \label{fig:ILP_analysis}

\end{figure*}


\textbf{Candidate architecture evaluation} plays an important role in LANA. This step finds the best architecture quickly out of the diverse candidates generated by the ILP solver, by evaluating them on 6k images from the train data. The procedure is built on the assumption that the accuracy of the model on the training data before finetuning (just by plugging all candidate operations) is a reasonable indicator of the relative model performance after finetuning. As shown in Fig.~\ref{fig:ILP_analysis}\subref{fig:ilp_vs_random}, when plugging pretrained operations into the teacher, the accuracy is high (it is above 30\%, even at an acceleration factor of 2$\times$). For EfficientNetV1, this is above 50\% for the same compression factor. 

% to appendix
% \input{tables/candidate_evaluation.tex}
% \textbf{Verifying pre/post finetuning model ranking.} We finetuned 31 models sampled from the pertained operations and measured their top-1 accuracy. The linear objective used in our ILP ranks those model architectures with a correlation score of 0.66 for Kendall Tau index and 0.85 for Spearman. When we measure the training accuracy of the candidate architecture before finetuning as the ranking indicator, the correlation is significantly improved to 0.835 for Kendall Tau index and 0.945 for Spearman. These observations are shown in Fig.~\ref{fig:ILP_analysis}\subref{fig:candidate_evaluation}.
% In Table~\ref{tab:candidate_evaluation_metrics}, we use different metrics to rank candidate architectures and observe that most correlates well with the final model accuracy after the finetuning.

\input{tables/nas_comparison.tex}
\textbf{Comparing with other NAS approaches.} We compare our search algorithm with other popular approaches to solve Eq.~(\ref{eq:nas_formulation}), including: (i) \textit{Random} architecture sampling within a latency constrain; (ii) \textit{Differentiable search with Gumbel Softmax} -- a popular approach in NAS to relax binary optimization as a continuous variable optimization via learning the sampling distribution~\citep{xie2018snas, Wu_2019_CVPR,vahdat2020unas}. We follow SNAS~\citep{xie2018snas} in this experiment; (iii) \textit{REINFORCE} is a stochastic optimization framework borrowed from reinforcement learning and adopted for architecture search~\citep{pham2018efficient, zoph2018learning,tan2019mnasnet}. We follow an E-NAS-like~\citep{pham2018efficient} architecture search for (iii) and use weight sharing for (ii) and (iii).
%Since both Gumbel Softmax and REINFORCE are compute and memory intensive, we only use the top 10 operations per layer, chosen based on high accuracy and low latency. 
Experiments are conducted on EfficientNetV1-B2 accelerated to 0.45$\times$ original latency. The final validation top-1 accuracy after finetuning are presented in Table~\ref{tab:nas_comparison}. Our proposed ILP achieves higher accuracy ($+0.43\%$) compared to the second best method E-NAS while being 821$\times$ faster in search. %. It is also faster by more than 820 times because no backpropagation is required and only a small portion (up 100) architectures are evaluated. % There are might be better NAS approaches, however we rely on a teacher model and can find reliable architectures within seconds or up to few minutes. 

\input{tables/only_skip}
\textbf{Zero-shot LANA.} Our method can be applied without pretraining procedure if only teacher cells and \textit{Identity} (skip) operation are used ($M=2$ operations per layer). Only the vector for the change in loss for the \textit{Identity} operator will be required alongside the LUT for the teacher operations. This allows us to do zero-shot network acceleration without any pretraining as reported in Table~\ref{tab:zero_shot_LANA}. We observe that LANA efficiently finds residual blocks that can be skipped. This unique property of LANA is enabled because of accelerating layers as apposed to blocks as done in \cite{Li_2020_CVPR, moons2020distilling}.
% by the search with ILP, and, to the best of our knowledge, no other NAS-based accelerating techniques are capable of zero-shot constrained NAS.

\textbf{Pretraining insights.} 
\label{sec:pretraining_insights}
To gain more insights into the tradeoff between the accuracy and speed of each operation, we analyze the pretrained candidate operation pool for EffientNetV1B2. %A detailed Figure~\ref{fig:phase2} is shown in the Appendix~\ref{sec:pretraining_app}, 
A detailed figure is shown in the appendix. Here, we provide general observations.

We observe that no operation outperforms the teacher in terms of accuracy; changing pretraining loss from per-layer MSE to full-student cross-entropy may change this but that comes with an increased costs of pretraining.
We also see that it is increasingly difficult to recover the teacher's accuracy as the depth in the network increases. The speedups achievable are roughly comparable across different depths, however, we note that achieving such speedups earlier in the network is particularly effective towards reducing total latency due to the first third of the layers accounting for 54\% of the total inference time.

Looking at individual operations, we observe that inverted residual blocks ({\small\texttt{efn}}, {\small \texttt{efnv2}}) are the most accurate throughout the network, at the expense of increased computational cost (\emph{i.e.,} lower speedups). Dense convolutions ({\small \texttt{cb\_stack}}, {\small \texttt{cb\_bottle}}, {\small \texttt{conv\_cs}}, {\small \texttt{cb\_res}}) exhibit a good compromise between accuracy and speed, with stacked convolutions being particularly effective earlier in the network.
%The identity operation unsurprisingly achieves very high speedups at the expense of increasingly poor accuracy compared to the teacher as a function of depth. 
Visual transformer blocks ({\small \texttt{ViT}}) and bottleneck transformer blocks ({\small \texttt{bot\_trans}}) show neither a speedup advantage nor are able to recover the accuracy of the teacher.

% \textbf{Common Operations.} In Appendix~\ref{fig:operators_distribution}, we analyze the distribution of the selected operations by solving for 100 architecture candidates with Eq.~\ref{eq:integer} for 0.5$\times$EfficientNetV1B2. We observe the following insights: (i) teacher operations are selected most frequently, it is expected as we only transform the model and no operations can beat teacher in terms of accuracy; 
% (ii) identity operation is selected more often for large architectures with higher compression rates;
% (iii) dense convolution blocks tend to appear more for larger models like EfficientNet-B6 to speed them up. 


\subsubsection{Architecture insights}

%Figures~\ref{fig:final_arch}-\ref{fig:final_arch3} 
In the appendices, we visualize the final architectures discovered by LANA. Next, we share the insights observed on these architectures. 

% \textbf{Common across all models:}  (i) Teacher's operations are usually selected in the tail of the network as they are relatively fast and approximating them results in the highest error. (ii) Teacher operation is preferred for downsampling layers (e.g. stride is 2). Those cells are hard to approximate as well, we hypothesize this is due to high nonlinearity of these blocks. (iii) Transformer blocks are never selected, probably because they 
% require significantly longer pretraining on larger datasets. (v) LANA automatically adjusts depth of every resolutional block by replacing teacher cells with Identity operations.

\textbf{EfficientNetV1.}
 Observing final architectures obtained by LANA on the EfficientNetV1 family, particularly the 0.55$\times$B2 version optimized for GPUs,  we discover that most of the modifications are done to the first half of the model: (i) squeeze-and-excitation is removed in the early layers; (ii) dense convolutions (like inverted stacked or bottleneck residual blocks) replace depth-wise separable counterparts; (iii) the expansion factor is reduced from 6 to 3.5 on average. \textit{Surprisingly, LANA automatically discovers the same design choices that are introduced in the EfficientNetV2 family when optimized for datacenter inference.} 

\textbf{EfficientNetV2.} LANA accelerates EfficientNetV2-B3 by 2$\times$, leading to the following conclusions: (i) the second conv-bn-act layer 
%\AV{layer or block?}\PM{layer, EFNV2 has 2 simple CBA in a row}
is not needed and can be removed; (ii) the second third 
% \AV{second and third block?}
of the model benefits from reducing the expansion factor from 4 to 1 without squeeze-and-excitation operations. With these simplifications, the accelerated model still outperforms EfficientNetV2-B2 and B1.

\textbf{ResNeST50.} LANA on ResNeST50d % \_1s4x24d 
discovers that cardinality can be reduced from 4 to 1 or 2 for most blocks without any loss in accuracy, yielding a 1.45$\times$ speedup.

\subsubsection{Ablations on finetuning}

% \input{tables/finetuning_study}

\hspace{1.9mm} \textbf{Pretrained weights.} We look deeper into the finetuning step. % to get intuition of different components. 
For this experiment, we select our 0.45$\times$EfficientNetV1-B2 with the final accuracy of 79.71\%. 
Reinitializing all weights in the model, as opposed to loading them from the pretraining stage, results in 79.42\%. The result indicates the importance of pretraining stage (i) to find a strong architecture and (ii) to boost finetuning.

\textbf{Knowledge distillation} plays a key role in student-teacher setups. When it is disabled, we observe an accuracy degradation of 0.65\%. This emphasizes the benefit of training a larger model and then distilling to a smaller one. We further verify whether we can achieve a similar high accuracy using knowledge distillation from EfficientNetV1-B2 to vanilla EfficientNetV1-B0 in the same setting. The top-1 accuracy of 78.72\% is still 1\% less than LANA's accuracy. 
When both models are trained from scratch with the distillation loss, LANA 0.45xB2 achieves 79.42\% while EfficientNetV1-B0 achieves 78.01\%. %We conclude that transforming the teacher into more efficient architecture is significantly more beneficial than fine-tuning smaller models. 
This verifies that results similar to LANA cannot be obtained simply by distilling knowledge from larger EfficientNets to smaller ones.

\input{tables/finetuning_length}
\textbf{Length of finetuning.} Pretrained operations have already been trained to mimic the teacher layer. Therefore, even before finetuning the student model can be already adept at the task. Next, we evaluate how does the length of finetuning affects the final accuracy in Table~\ref{tab:finetuning_length}. Even with only 5 epochs LANA outperforms the vanilla EfficientNet counterparts.

\input{tables/search_space}

\textbf{Search space size.} ILP enables us to perform NAS in a very large space ($O(10^{100})$). To verify the benefit of large search space, we experiment with a restricted search space. For this, we randomly pick 2, 5 and 10 operations per layer to participate in search and finetuning for 50 epochs. We observe clear improvements from increasing the search space, shown Table~\ref{tab:search_space} (results are averaged over 5 runs).   

\input{tables/donna_table}
\textbf{Comparison to~\cite{moons2020distilling}.} DONNA has a similar motivation ours and has reported results comparable to our setup. We observe significant improvements over DONNA in the Table~\ref{tab:donna_comparison} with lower latency and higher accuracy.

==> LANA_CVPR2022_arxiv%20(Version%20281)/2_experiments.tex <==
\vspace{-0.1cm}
\section{Experiments}
\vspace{-0.1cm}
\label{sec:experiments}


We apply LANA to the family of EfficientNetV1~\citep{tan2019efficientnet}, EfficientNetV2~\citep{tan2021efficientnetv2} and ResNeST50~\citep{zhang2020resnest}. When naming our models, we use the latency reduction ratio compared to the original model according to latency look-up table (LUT). For example, 0.25$\times$B6 indicates 4$\times$ target speedup for the B6 model.

For experiments, ImageNet-1K~\citep{ILSVRC15} is used for pretraining (1 epoch), candidate evaluation (6k training images) and finetuning (100 epochs). 
 

We use the NVIDIA V100 GPU and Intel Xeon Silver 4114 CPU as our target hardware. A hardware specific look-up table is precomputed for each candidate operation (vectors $\mathbf{b}_i$ in Eq.~\ref{eq:integer}). 
We measure latency in 2 settings: (i) in Pytorch framework, and (ii) TensorRT ~\citep{tensorrt}. The latter performs kernel fusion for additional model optimization making it even harder to accelerate models. Note that the exact same setup is used for evaluating latency of \textbf{all} competing models, our models, and baselines.  Actual latency on the target platform is reported in the tables.  

\textbf{Candidate operations. } 
We construct a large of pool of diverse candidate operation including $M=197$ operations for each layer of teacher. 
Our operations include:

{\parskip=2pt
\begin{itemize}[topsep=1pt,itemsep=1pt,partopsep=0pt,parsep=0pt,leftmargin=0pt]

\item[]\underline{Teacher operation} is used as is in the pretrained model with teacher model accuracy.

\item[]\underline{Identity} is used to skip teacher's operation. It changes the depth of the network. 

\item[]\underline{Inverted residual blocks} \texttt{efn} \citep{sandler2018mobilenetv2} and \texttt{efnv2} \citep{tan2021efficientnetv2}  with varying expansion factor $e{=}\{1,3,6\}$, squeeze and excitation ratio $se{=}\{\textrm{No}, 0.04, 0.025\}$, and kernel size $k{=}\{1, 3, 5\}$. 

\item[]\underline{Dense convolution blocks} inspired by~\cite{he2016identity} with (i) two stacked convolution (\texttt{cb\_stack}) with CBRCB structure, C-conv, B-batchnorm, R-Relu; (ii) bottleneck architecture (\texttt{cb\_bottle}) with CBR-CBR-CB; (ii) CB pair (\texttt{cb\_res}); (iii) RepVGG block~\citep{ding2021repvgg}; (iv) CBR pairs with perturbations as \texttt{conv\_cs}. For all models we vary kernel size $k = \{1,3,5,7\}$ and width $w = \{1/16, 1/10, 1/8, 1/5, 1/4, 1/2, 1, 2, 3, 4\}$.

\item[]\underline{Transformer variations} (i) visual transformer block~(\texttt{vit}) \citep{dosovitskiy2020image} with depth $d=\{1,2\}$, dimension $w=\{2^5, 2^6, 2^7, 2^8, 2^9, 2^{10}\}$ and heads $h=\{4,8,16\}$; (ii) bottleneck transformers~\citep{srinivas2021bottleneck} with 4 heads and expansion factor $e = \{1/4, 1/2, 1, 2, 3, 4\}$; (iii) lambda bottleneck layers~\citep{bello2021lambdanetworks} with expansion $e=\{1/4, 1/2, 1, 2, 3, 4\}$. 
\end{itemize}
}

\input{tables/gpu_results_cvpr}

With the pool of 197 operations, distilling from an EfficientNet-B6 model with $46$ layers yields a design space of the size \(197^{46}\!\approx\!10^{100}\). 


\subsection{EfficientNet and ResNeST Derivatives}

Our experimental results on accelerating EfficientNetV1(B2, B4, B6), EfficientNetV2(B3), and ResNeST50 family for GPUs are shown in Table~\ref{tab:imagenet_comparison} and Figure~\ref{fig:imagenet_comparison}.
Comparison with more models from \texttt{timm} is in the Appendix. 

\textbf{Results demonstrate that: }
% We make the following observations:
{\parskip=2pt
\begin{itemize}[topsep=1pt,itemsep=1pt,partopsep=0pt,parsep=0pt,leftmargin=10pt]
% \item[]We make the following observations:
\item LANA achieves an \textbf{accuracy boost of} $\mathbf{0.18-3.0}\%$ for all models  when compressing larger models to the latency level of smaller models (see EfficientNet models and the corresponding LANA models in the same latency group).
\item LANA achieves \textbf{significant real speed-ups} with little to no accuracy drop: 
(i) Efficiei87ntNetV1-B6 accelerated by 3.6x and 1.8x times by trading-off 0.34\% and 0.11\% accuracy, respectively; (ii) B2 variant is accelerated 2.4x and 1.9x times with 0.36\% and no accuracy loss, respectively. (iii) ResNeST50 is accelerated 1.5x with 0.84\% accuracy drop.
\end{itemize}
}

A detailed look on EfficientNets is shown in Figure~\ref{fig:imagenet_comparison}, where we observe that EfficientNetV1 models are accelerated beyond EfficientNetV2. LANA generates models that have better accuracy-throughput trade-off when comparing models under the same accuracy or the same latency. LANA also allows us to optimize models for different hardware at a little cost. Only a new LUT is required to get optimal model for a new hardware without pretraining the candidate operations again. We present models optimized for CPU in Table~\ref{tab:efficientnetv1_cpu} which are obtained using a different LUT.  

% \textbf{Throughput} is significantly improved with LANA, making EfficientNets up to $2\times$ faster (EfficientNetV1-B3 vs.\ 0.25$\times$B4). EfficientNetV1s are accelerated beyond original EfficientNetV2. ResNeST50 is accelerated by 1.5$\times$ with only 0.14\% drop in accuracy.

% \textbf{Accuracy} is also significantly higher compared to the models with the same latency. Our 0.25$\times$B4 obtains 3.0\% higher top-1 accuracy compared to the original EfficientNetV1-B1 while maintaining a similar latency. EfficientNetV2-B3 accelerated by 1.7$\times$ gains $0.93\%$ with respect to EfficientNetV2-B2. Trade-off between accuracy and latency is obtained by accelerating EfficientNet models by up to 3.6$\times$ while scarifying only $0.3\%$ accuracy as for the 0.25$\times$B6 variant.

% As observed in Table~\ref{tab:imagenet_comparison}, we apply LANA to a large spectrum of model sizes on two different target hardware types. This is possible in LANA due to (i) independent and fully parallel layer-wise distillation, (ii) separating search from pretraining stage, and hence alleviating the need to retrain candidate operations before optimizing a network for a new hardware, and (iii) using a light-weight linear optimization for architecture search that allows for efficient and effective searching in a large architecture space.  

\input{tables/cpu_results}



==> LANA_CVPR2022_arxiv%20(Version%20281)/3_ack.tex <==
\section*{Acknowledgement}
This work was conducted jointly at NVIDIA and Microsoft research. The authors would like to thank Azure ML and the office of the CTO at Microsoft as well as the NVIDIA NGC team for compute support.



==> LANA_CVPR2022_arxiv%20(Version%20281)/broader_impact.tex <==

\subsection{Analysis}

\input{tables/cpu_restable_wrap}
All studies in this section are performed with the setting of compressing  EfficientNet-B2 by $0.45\times$ to match the latency of B0. Finetuning is reduced to 50 epochs only, while search is limited to 50 architectures. Additional ablation studies on the length of pretraining, contribution of distillation loss for finetuning, and importance of pre-loading weights can be found in Appendix.

\textbf{Pretraining Stage.}
To gain more insights into the tradeoff between the accuracy and speed of each operation, we analyze the the pretrained candidate operation pool. Figure~\ref{fig:phase2} highlights tradeoff for three layers spaced equally throughout the network. In general,
we observe that no operation outperforms the teacher in terms of accuracy.
We also see that it is increasingly difficult to recover the teacher's accuracy as the depth in the network increases. For example, the best operation at layer 7 can recover around 100\% of the teacher's performance, whereas it drops to 99\% by layer 21. The speedups achievable are roughly comparable across different depths, however we note that achieving such speedups earlier in the network is particularly effective towards reducing total latency due to the first third of the layers accounting for 54\% of the total inference time. 

Looking at individual operations, we observe that inverted residual blocks (\texttt{efn}, \texttt{efnv2}) are the most accurate throughout the network, at the expense of increased computational cost (\emph{i.e.,} lower speedups). Dense convolutions (\texttt{cb\_stack}, \texttt{cb\_bottle}, \texttt{conv\_cs}, \texttt{cb\_res}) exhibit a good compromise between accuracy and speed, with stacked convolutions being particularly effective earlier in the network (\emph{e.g.,} see 7$^\text{th}$ layer). The identity operation unsurprisingly achieves very high speedups at the expense of increasingly poor accuracy compared to the teacher as a function of depth. Visual transformer blocks (\texttt{ViT}) and bottleneck transformer blocks (\texttt{bot\_trans}) show neither a speedup advantage nor are able to recover the accuracy of the teacher. Indeed, their performance, across all axes, gets progressively worse as a function of depth, and as a result they are never selected during the search.



\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth,trim=.25cm .25cm .25cm .25cm,clip=true]{images/pretraining_efnb2_3layers.pdf}
    \caption{Result of the pretraining stage for EfficientNetB2, showing three layers equally spaced throughout the network: 7, 14 and 21. Speedup is measured as the ratio between the latency of the teacher and the latency of the student operation (higher is better). We measure latency using Pytorch FP16. Accuracy is the ratio of the operation's accuracy and the teacher's (higher is better). The dashed black lines correspond to the teacher.} 
    \label{fig:phase2}
\end{figure}

\textbf{Architecture Search.}
We compare our implementation of architecture search with other popular approaches to solve Eq.~(\ref{eq:nas_formulation}), including: (i) \textit{Random} architecture sampling within a latency constrain; (ii) \textit{Differentiable search with Gumbel Softmax} -- a popular approach in NAS to relax binary optimization as a continuous variable optimization via learning the sampling the distribution~\cite{xie2018snas, Wu_2019_CVPR,vahdat2020unas}. We follow SNAS~\cite{xie2018snas} in this experiment; (iii) \textit{REINFORCE} is a stochastic optimization framework borrowed from reinforcement learning and adopted for architecture search~\cite{pham2018efficient, zoph2018learning,tan2019mnasnet}. We follow an E-NAS-like~\cite{pham2018efficient} architecture search. Both learning-based solutions (ii) and (iii) benefit from simultaneous architecture and weight tuning, therefore we do search with and without those updates. Since both Gumbel Softmax and REINFORCE are compute and memory intensive, we only use the top 10 operations per layer, chosen based on high accuracy and low latency. 

Different variations of NAS are compared in Table~\ref{tab:ablation}. We make the following observations: (i) the proposed integer optimization for search significantly outperforms Gumbel Softmax and REINFORCE while being orders of magnitude faster in search; (ii) Both Gumbel Softmax and REINFORCE perform poorly when weights are not initialized using our pretraining phase, emphasizing on the importance of phase one. (iii) The substantial improvement is obtained with increasing number of candidate operations for integer optimization while Gumbel Softmax and REINFORCE cannot handle large number of operations; (iv) there is a strong correlation between the loss after search on training set with the final one on the validation set; (v) the search and evaluation costs are significantly lower for integer optimization; (vi) final accuracy increases with increasing the number of candidate architectures $k$ for linear optimization. Accuracy correlation before and after search allows us to evaluate candidates without training candidate architectures, performing search at minimal cost. 

\input{tables/nas_comparison.tex}


\textbf{Common Operations.} In Appendix, we analyse the distribution of the selected operations by solving for 100 architecture candidates with Eq.~\ref{eq:integer} and picking the top-10 of them. We observe the following insights: (i) teacher operations are selected most frequently, it is expected as we only transform the model and no operations can beat teacher in terms of accuracy; 
(ii) identity operation is selected more often for architectures with higher compression rates versus small compression;
(iii) dense convolution blocks tend to appear more for larger models like EfficientNet-B6 to speed them up. 


\textbf{Final Architectures.} We analyze final architectures (detailed structures in Appendix) and observe: (i) Teacher's operations are usually selected in the tail of the network as they are relatively fast and approximating them results in the highest error. (ii) Teacher operation is preferred for downsampling layers (e.g. stride is 2). Those cells are hard to approximate as well. (iii) Transformer blocks are never selected, probably because they 
require significantly longer pretraining on larger datasets. (iv) As the networks get larger, we see more dense convolutions being selected rather than depth-wise separable counterparts. (v) Identity operations are more often seen in the first half of the network for architectures when we want to achieve high compression. 


\begin{wrapfigure}{r}{0.35\textwidth}
    \vspace{-0.5cm}
    \includegraphics[width=0.99\textwidth, trim={0.25cm 0.25cm 0.25cm 0.25cm},clip]{images/compression_vs_final_acc.pdf}
    \vspace{-0.7cm}
    \caption{\small Accuracy vs. compression}
    % \vspace{-0.65cm}
    \label{fig:train_vs_va}
\end{wrapfigure}

\textbf{Compression / Accuracy Trade-off.} Compressing any given network with different rates will produce a family of accelerated networks. However, accuracy will starts decreasing with aggressive compression rates. We demonstrate this effect in Figure~\ref{fig:train_vs_va}, where we see a sharp drop in accuracy with compression rates below $0.3$. It can be explained by a weak prior on accuracy used in our linear optimization to characterize non-linear dynamics of networks, which in turn makes our relaxation a poor approximation of the actual loss.

==> LANA_CVPR2022_arxiv%20(Version%20281)/final_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}
% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See the \textbf{Limitation} section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We included detailed discussions on the associated computation in GPU hours as required by HANT. We also include additional discussion in the \textbf{Broader Impact} section.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA
	\item Did you include complete proofs of all theoretical results?
    \answerNA
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include code and HANT-based ImageNet EfficientNet Derivatives in supplemental materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Sec.~\ref{sec:experiments}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We did not repeat NAS runs amid high GPU computation requirement when combining both phases in overall pipeline. We report error bars for latency measurements.} \DY{PLEASE CHECK - UPDATE after experiments.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We included detailed descriptions of each computation environment alongside our experiments.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets... 
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite relevant creators/datasets in both the main paper and the Appendix.} 
  \item Did you mention the license of the assets?
    \answerYes{We mention the license of the assets in Appendix.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We used publicly available assets and did not introduce new ones.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{All datasets we used are publicly available and we specified the dataset names in experiments.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects in this paper.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects in this paper.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects in this paper.}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> LANA_CVPR2022_arxiv%20(Version%20281)/images/figure_architectures.tex <==
\begin{figure*}
 \centering    
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[height=.7\textheight]{images/graph_0.45xB2.pdf}
         \caption{0.45xB2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[height=.7\textheight]{images/graph_0.55xB2.pdf}
         \caption{0.55xB2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[height=.9\textheight]{images/graph_0.25xB6.pdf}
         \caption{0.25xB6}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[height=.9\textheight]{images/graph_0.50xB6.pdf}
         \caption{0.5xB6}
     \end{subfigure}
     \vspace{1cm}
        \caption{Final architectures selected by LANA  as EfficientNet-B2/B6 derivatives.}
        \label{fig:final_arch}
\end{figure*}


\begin{figure*}
\centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[height=.9\textheight]{images/graph_0.2xB4.pdf}
         \caption{0.2xV1-B4}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[height=.9\textheight]{images/graph_0.25xB4.pdf}
         \caption{0.25xV1-B4}
     \end{subfigure}
          \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[height=.9\textheight]{images/graph_0.3xB4.pdf}
         \caption{0.3xV1-B4}
     \end{subfigure}
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[height=.9\textheight]{images/graph_0.5xB4.pdf}
         \caption{0.5xV1-B4}
     \end{subfigure}
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[height=.9\textheight]{images/graph_V2B3x0.50.pdf}
         \caption{0.5xV2-B3}
     \end{subfigure}     
     \vspace{1cm}
        \caption{Final architectures selected by LANA  as EfficientNetV1-B4/V2-B3 derivatives.}
        \label{fig:final_arch2}
\end{figure*}




\begin{figure*}
\centering
\includegraphics[width=.9\textwidth]{images/graph_0.7xResNeST.pdf}

\caption{Final architectures selected by LANA  as 0.7xResNeST50d\_1s4x24d}
\label{fig:final_arch3}
\end{figure*}

==> LANA_CVPR2022_arxiv%20(Version%20281)/images/figure_ops_distribution.tex <==
\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/ops_selected_analysis_0.45xB2_0.55xB2.pdf}
         \caption{B2 selected ops}
         \label{fig:ops_b2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/ops_selected_analysis_0.3xB4_0.5xB4.pdf}
         \caption{B4 selected ops}
         \label{fig:ops_b4}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/ops_selected_analysis_0.2xB4_0.25xB4.pdf}
         \caption{B4 selected ops}
         \label{fig:ops_b6}
     \end{subfigure}
     \vspace{1cm}
        \caption{The histogram of selected operations for top-100 models of EfficientNetV1 derivatives. Teacher layers are often selected especially in the deeper layers of the network as we visualize in Fig.~\ref{fig:final_arch} and Fig.~\ref{fig:final_arch2}. The identity layer is also selected often especially when the target latency is low. Interestingly, simple layers with two stacked convolution (\texttt{cb\_stack}) in the CBRCB structure (C-convolution, B-batchnorm, R-ReLU) are selected most frequently after the teacher and identity operations. Additionally we see a higher chance of selecting inverted residual blocks (\texttt{efn} and \texttt{efn2}) with no squeeze-and-excitation operations \texttt{se1.00}. }
        \label{fig:operators_distribution}
\end{figure*}

==> LANA_CVPR2022_arxiv%20(Version%20281)/images/imagenet_gpu.tex <==
\begin{figure}[t]
     \centering
     \includegraphics[width=0.45\textwidth, trim={0cm 0 0cm 0cm},clip]{images/v2/efn_plot.pdf}
     \caption{A visual summary of the EfficientNetV1 and EfficientNetV2 model families accelerated by LANA. Accelerated EfficientNetV1 models outperform EfficientNetV2 models.}
     \label{fig:imagenet_comparison}
 \end{figure}

==> LANA_CVPR2022_arxiv%20(Version%20281)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/candidate_evaluation.tex <==
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\vspace{0cm}
\vspace{0mm}
\caption{\small Candidate evaluation metrics for model ranking before and after finetuning. \vspace{-0.0cm}} \label{tab:candidate_evaluation_metrics}
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Correlation & Accuracy & Cross-entropy & KL divergence & MSE \\
\midrule
Kendal Tau  & 0.835 & 0.824 & 0.832 & 0.811 \\
Spearman    & 0.945 & 0.947 & 0.954 & 0.944\\ 
\bottomrule \vspace{-0.0cm}
\end{tabular}
}
% \vspace{-8mm}
\end{table}
%\vspace{-0.3cm}

% kdt, 0.772, spearman, 0.914
% metric:  eval_loss
% kdt, 0.776, spearman, 0.924
% metric:  eval_kdloss
% kdt, 0.673, spearman, 0.843
% metric:  eval_mseloss
% kdt, 0.475, spearman, 0.647

% metric:  train_accuracy
% kdt, 0.835, spearman, 0.945
% metric:  train_loss
% kdt, 0.824, spearman, 0.947
% metric:  train_kdloss
% kdt, 0.832, spearman, 0.954
% metric:  train_mseloss
% kdt, 0.811, spearman, 0.944

==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/cpu_results.tex <==
 \begin{table}[b]
  \centering
  \caption{EfficientNetV1 accelerated by LANA for CPU inference.}
  \vspace{-0.2cm}
    \resizebox{0.4\textwidth}{!}{%
    \begin{tabular}{lclc}
        \toprule
        \multirow{2}{*}{Model} & Res. & Accuracy & Latency \\
         & (px) & (\%) & Pytorch (ms) \\
        \midrule
        \midrule
        EfficientNetB0          & 224  & 77.70 & 57\\
        0.4xB2 (Xeon)           & 260 & 78.11 (+0.97) & 48 \\
        0.5xB2 (Xeon)           & 260 & 78.87 (+1.17) & 58  \\
        \midrule
        EfficientNetB1          & 240 & 78.83 & 86\\
        0.7xB2 (Xeon)           & 260 & 79.89 (+1.06) & 80 \\
        \midrule
        EfficientNetB2          & 260 & 80.07 & 113\\
        \bottomrule
    \end{tabular}
    }%
  \label{tab:efficientnetv1_cpu}
 \end{table}

==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/donna_table.tex <==
\begin{table}[t]
  \caption{Comparison to \cite{moons2020distilling}. Latency values measured on V100 GPU at batch size $32$ with PyTorch FP32. All models were finetuned for 50 epochs only. }
  \label{tab:donna_comparison}
  \vspace{-0.2cm}
  \centering
  \resizebox{0.4\textwidth}{!}{
  \begin{tabular}{lcc}
    \toprule
    \multicolumn{1}{c}{Models}   & Latency    & Top-1 Acc.     \\
             & (ms) $\downarrow$ &  ($\%$) $\uparrow$ \\
    \midrule
    DONNA~\cite{moons2020distilling} & $20.0$ & $78.9$ \\
    \textbf{LANA} (0.45xEfficientNetV1-B2)  & \textbf{18.9} & \textbf{79.58 (+0.68)}  \\
    \midrule
    DONNA~\cite{moons2020distilling} & 25.0 & 79.5 \\
    \textbf{LANA} (0.55xEfficientNetV1-B2) & \textbf{24.1} & \textbf{80.0 (+0.5)}\\
    \bottomrule
  \end{tabular}
  }
  \vspace{-0pt}
\end{table}



==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/finetuning_length.tex <==
\begin{table}
    \centering
    \setlength{\tabcolsep}{3pt}
    

\caption{{Ablations on the length of finetuning step. On the right side, we report EfficientNet accuracy for models with the same latency as ours.} \vspace{-0.0cm}}
\vspace{-.2cm}
\label{tab:finetuning_length}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{x{1.5cm}x{1.2cm}x{1.2cm}x{1.2cm}x{1.2cm}x{1.2cm}|x{2.0cm}}
\toprule
LANA  &  \multicolumn{5}{c|}{Epochs} & \small{EfficientNetV1} \\ \cline{2-6}
model &   5 & 10 & 25 & 50 & 100 & alternative\\ \hline
% \middlerule
 0.45xB2  &78.69 & 79.08 & 79.19 &	79.58 &	79.71 & 77.70 (B0) \\ 
 0.55xB2  & 79.05 & 79.47 & 79.84 &	80.00 &	80.11 & 78.83 (B1)\\
\bottomrule
\end{tabular}}
\end{table}


==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/gpu_results.tex <==
    \begin{table}[h]
    \centering
    \caption{CPU optimized models:} 
    \label{tab:cpu_results}
    \resizebox{0.4\textwidth}{!}{%
    
    \begin{tabular}{lclc}
    \toprule
    \multirow{2}{*}{Model} & Res. & Accuracy & Latency \\
     & (px) & (\%) & Pytorch (s) \\
    \midrule
    \midrule
    EfficientNetB0          & 224  & 77.70 & 0.057 $\pm$ 0.001  \\
    0.4xB2 (Xeon)           & 260 & 78.11 (+0.97) & 0.048 $\pm$ 0.001 \\
    0.5xB2 (Xeon)           & 260 & 78.87 (+1.17) & 0.058 $\pm$ 0.001 \\
    \midrule
    EfficientNetB1          & 240 & 78.83 & 0.086 $\pm$ 0.001 \\
    0.7xB2 (Xeon)           & 260 & 79.89 (+1.06) & 0.080 $\pm$ 0.001 \\
    \midrule
    EfficientNetB2          & 260 & 80.39 & 0.113 $\pm$ 0.002 \\
    \bottomrule
    \end{tabular}
    }
    \end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth, trim={0cm 0 1cm 1cm},clip]{images/v2/effnv2.pdf}
    \caption{EfficientNets compression with HANT for V100 GPU:}
    \label{fig:result_efn_plot}
\end{figure}

\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.4\textwidth}{!}{%
    \begin{tabular}{lclcc}
    \toprule
    \multirow{2}{*}{Model} & Res & Accuracy & \multicolumn{2}{c}{Latency(ms) per 128 images} \\
     & {px} & (\%)  & TensorRT & PyTorch\\
    \midrule
    \midrule
    \multicolumn{5}{c}{\textbf{EfficientNetV1}}  \\
    \midrule
    \midrule
    EfficientNetV1-B0         & 224  & 77.70 & 17.9 & 35.6 \\
    0.45xB2                & 260  & \textbf{79.71 (+2.01)} & \textbf{16.2} & 30.2\\      
    \midrule
    EfficientNetV1-B1         & 240  & 78.83 & 29.3 & 59.0 \\
    0.55xB2                & 260  & 80.11 (+1.28) & \textbf{20.6} & 48.7\\      
    0.2xB4                 & 380  & 80.33 (+1.50) & 33.0 & 64.5\\
    0.25xB4                 & 380  & \textbf{81.83 (+3.00)} & 30.4 & 64.5\\
    \midrule
    EfficientNetV1-B2         & 260  & 80.39 & 38.2 & 77.1 \\
    0.3xB4                 & 380  & \textbf{82.16 (+1.77)} & \textbf{38.8} & 81.8\\        
    \midrule
    EfficientNetV1-B3         & 300  & 81.67 & 67.2 & 125.9 \\
    0.5xB4                 & 380  & \textbf{82.66 (+0.99)} & \textbf{61.4} & 0.1914\\            
    \midrule
    EfficientNetV1-B4         & 380  & 83.02 & 132.0 & ?  \\
    % 0.2xB6               & 528  & 82.57 & \textbf{0.1515} & 0.3243 & 0.5654 \\
    0.25xB6                & 528  & \textbf{83.77 (+0.75)} &  \textbf{128.8} & ?\\
    \midrule
    EfficientNetV1-B5         & 456  & 83.81 & 265.7 & ?  \\
    % 0.45xB6                & 528  & \textbf{83.85 (+0.04)} & \textbf{0.3560} & 0.7261\\
    0.5xB6                 & 528  & \textbf{83.99 (+0.18)} & \textbf{266.5} & ? \\
    \midrule
    EfficientNetV1-B6         & 528  & 84.11 & 466.7 & ?  \\
        \midrule
    \midrule
    \multicolumn{5}{c}{\textbf{EfficientNetV2}}  \\
    \midrule
    \midrule
    EfficientNetV2-B1         & 240  & 79.46 & 17.9 & 44.7 \\
    0.45xB3                   & 300  & \textbf{80.30 (+0.84)} & \textbf{17.8} & 43.0\\      
    \midrule
    EfficientNetV2-B2         & 260  & 80.21 & 24.3 & 58.9 \\
    0.6xB3                    & 300  & \textbf{81.14 (+0.93)} & \textbf{23.8} & 56.1\\      
    \midrule
    EfficientNetV2-B3       & 300  & 81.97 & 41.2 & 91.6 \\
    \midrule
    \midrule
    \multicolumn{5}{c}{\textbf{ResNeST50d\_1s4x24d}}  \\
    \midrule
    \midrule
    ResNeST50       & 224  & 80.99 & 32.3 & 74.0 \\
    0.7x            & 224  & 80.85 & \textbf{22.3(1.45x)} & 52.7 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Models optimized for GPU inference}
    \label{tab:gpu_results}
\end{table}


==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/gpu_results_cvpr.tex <==
\begin{table}[t]
\centering
    \renewcommand{\arraystretch}{0.65}
    \setlength{\tabcolsep}{3pt}
    \centering
    % \footnotesize{GPU optimized models:}
        \caption{Models optimized with LANA for GPU inference, evaluated on ImageNet-1K. Latency is computed for a batch of 128 images over 10 runs on the actual hardware. Models are grouped by the latency to demonstrate accuracy improvement over the vanilla EfficientNet models with default model scaling.}
        
    \resizebox{0.49\textwidth}{!}{%
    \begin{tabular}{p{2.4cm}u{1.4cm}x{1.1cm}lcc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Variant} & Res & Accuracy & \multicolumn{2}{c}{Latency(ms)} \\
     & & {px} & (\%)  & TensorRT & PyTorch\\
    \midrule
    \midrule
    \multicolumn{6}{c}{\textbf{EfficientNetV1}}  \\
    \midrule
    \midrule
    EfficientNetV1 & 1.00xB0         & 224  & 77.70 & 17.9 & 35.6 \\
    LANA  & 0.45xB2                & 260  & \textbf{79.71 (+2.01)} & \textbf{16.2} & \textbf{30.2}\\      
    \midrule
    EfficientNetV1 & 1.00xB1         & 240  & 78.83 & 29.3 & 59.0 \\
    LANA & 0.55xB2                  & 260  & 80.11 (+1.28) & \textbf{20.6} & \textbf{48.7}\\      
    LANA & 0.20xB4                & 380  & 80.33 (+1.50) & 33.0 & 52.2\\
    LANA & 0.25xB4                 & 380  & \textbf{81.83 (+3.00)} & 30.4 & 64.5\\
    \midrule
    EfficientNetV1 & 1.0xB2         & 260  & 80.07 & 38.2 & 77.1 \\
    LANA & 0.3xB4                 & 380  & \textbf{82.16 (+2.09)} & \textbf{38.8} & 81.8\\        
    \midrule
    EfficientNetV1 & 1.0xB3         & 300  & 81.67 & 67.2 & 125.9 \\
    LANA  & 0.5xB4                & 380  & \textbf{82.66 (+0.99)} & \textbf{61.4} & 148.1\\            
    \midrule
    EfficientNetV1 & 1.00xB4         & 380  & 83.02 & 132.0 & 262.4  \\
    % 0.2xB6               & 528  & 82.57 & \textbf{0.1515} & 0.3243 & 0.5654 \\
    LANA & 0.25xB6               & 528  & \textbf{83.77 (+0.75)} &  \textbf{128.8} & 282.1\\
    \midrule
    EfficientNetV1 & 1.0xB5         & 456  & 83.81 & 265.7 & 525.6  \\
    % 0.45xB6                & 528  & \textbf{83.85 (+0.04)} & \textbf{0.3560} & 0.7261\\
    LANA &0.5xB6               & 528  & \textbf{83.99 (+0.18)} & \textbf{266.5} & 561.2 \\
    \midrule
    EfficientNetV1 & 1.0xB6         & 528  & 84.11 & 466.7 & 895.2  \\
        \midrule
    \midrule
    \multicolumn{6}{c}{\textbf{EfficientNetV2}}  \\
    \midrule
    \midrule
    EfficientNetV2 & 1.00xB1         & 240  & 79.46 & 17.9 & 44.7 \\
    LANA & 0.45xB3                  & 300  & \textbf{80.30 (+0.84)} & \textbf{17.8} & \textbf{43.0}\\      
    \midrule
    EfficientNetV2 & 1.0xB2         & 260  & 80.21 & 24.3 & 58.9 \\
    LANA & 0.6xB3                    & 300  & \textbf{81.14 (+0.93)} & \textbf{23.8} & \textbf{56.1}\\      
    \midrule
    EfficientNetV2 & 1.0xB3       & 300  & 81.97 & 41.2 & 91.6 \\
    \midrule
    \midrule
    \multicolumn{6}{c}{\textbf{ResNeST50d\_1s4x24d}}  \\
    \midrule
    \midrule
    ResNeST50 & 1.0x       & 224  & 80.99 & 32.3 & 74.0 \\
    LANA & 0.7x      & 224  & 80.85 & \textbf{22.3(1.45x)} & \textbf{52.7} \\
    \bottomrule
    \end{tabular}
    }%
    
     \centering
     \includegraphics[width=0.45\textwidth, trim={0cm 0 0cm 0cm},clip]{images/v2/efn_plot.pdf}
     \captionof{figure}{A visual summary of the EfficientNetV1 and EfficientNetV2 model families accelerated by LANA. Accelerated EfficientNetV1 models outperform EfficientNetV2 models.}
     \label{fig:imagenet_comparison}
    % \vspace{-.3cm}
    \label{tab:imagenet_comparison}
\end{table}




%\begin{table}[t]
% \centering
%     \renewcommand{\arraystretch}{0.65}
%     \setlength{\tabcolsep}{3pt}
%     \centering
%     % \footnotesize{GPU optimized models:}
%         \caption{Models optimized with LANA for GPU inference, evaluated on ImageNet-1K. Latency is computed for a batch of 128 images over 10 runs on the actual hardware. Models are grouped by the latency to demonstrate accuracy improvement over the vanilla models with default scaling.}
        
%     \resizebox{0.4\textwidth}{!}{%
%     \begin{tabular}{lclcc}
%     \toprule
%     \multirow{2}{*}{Model} & Res & Accuracy & \multicolumn{2}{c}{Latency(ms)} \\
%      & {px} & (\%)  & TensorRT & PyTorch\\
%     \midrule
%     \midrule
%     \multicolumn{5}{c}{\textbf{EfficientNetV1}}  \\
%     \midrule
%     \midrule
%     EfficientNetV1-B0         & 224  & 77.70 & 17.9 & 35.6 \\
%     LANA (0.45xB2)                & 260  & \textbf{79.71 (+2.01)} & \textbf{16.2} & \textbf{30.2}\\      
%     \midrule
%     EfficientNetV1-B1         & 240  & 78.83 & 29.3 & 59.0 \\
%     LANA (0.55xB2)                 & 260  & 80.11 (+1.28) & \textbf{20.6} & \textbf{48.7}\\      
%     LANA (0.2xB4)               & 380  & 80.33 (+1.50) & 33.0 & 52.2\\
%     LANA (0.25xB4)                & 380  & \textbf{81.83 (+3.00)} & 30.4 & 64.5\\
%     \midrule
%     EfficientNetV1-B2         & 260  & 80.07 & 38.2 & 77.1 \\
%     LANA (0.3xB4)                & 380  & \textbf{82.16 (+2.09)} & \textbf{38.8} & 81.8\\        
%     \midrule
%     EfficientNetV1-B3         & 300  & 81.67 & 67.2 & 125.9 \\
%     LANA (0.5xB4))                & 380  & \textbf{82.66 (+0.99)} & \textbf{61.4} & 148.1\\            
%     \midrule
%     EfficientNetV1-B4         & 380  & 83.02 & 132.0 & 262.4  \\
%     % 0.2xB6               & 528  & 82.57 & \textbf{0.1515} & 0.3243 & 0.5654 \\
%     LANA (0.25xB6)               & 528  & \textbf{83.77 (+0.75)} &  \textbf{128.8} & 282.1\\
%     \midrule
%     EfficientNetV1-B5         & 456  & 83.81 & 265.7 & 525.6  \\
%     % 0.45xB6                & 528  & \textbf{83.85 (+0.04)} & \textbf{0.3560} & 0.7261\\
%     LANA (0.5xB6)               & 528  & \textbf{83.99 (+0.18)} & \textbf{266.5} & 561.2 \\
%     \midrule
%     EfficientNetV1-B6         & 528  & 84.11 & 466.7 & 895.2  \\
%         \midrule
%     \midrule
%     \multicolumn{5}{c}{\textbf{EfficientNetV2}}  \\
%     \midrule
%     \midrule
%     EfficientNetV2-B1         & 240  & 79.46 & 17.9 & 44.7 \\
%     0.45xB3 (LANA)                  & 300  & \textbf{80.30 (+0.84)} & \textbf{17.8} & \textbf{43.0}\\      
%     \midrule
%     EfficientNetV2-B2         & 260  & 80.21 & 24.3 & 58.9 \\
%     0.6xB3 (LANA)                    & 300  & \textbf{81.14 (+0.93)} & \textbf{23.8} & \textbf{56.1}\\      
%     \midrule
%     EfficientNetV2-B3       & 300  & 81.97 & 41.2 & 91.6 \\
%     \midrule
%     \midrule
%     \multicolumn{5}{c}{\textbf{ResNeST50d\_1s4x24d}}  \\
%     \midrule
%     \midrule
%     ResNeST50       & 224  & 80.99 & 32.3 & 74.0 \\
%     0.7x (LANA)     & 224  & 80.85 & \textbf{22.3(1.45x)} & \textbf{52.7} \\
%     \bottomrule
%     \end{tabular}
%     }%

%     % \vspace{-.3cm}
%     \label{tab:imagenet_comparison}
% \end{table}
 
 
 

%   \begin{minipage}[b]{0.55\textwidth}
%   \centering
%   \begin{tabular}{c}
%   % \footnotesize{EfficientNets acceleration with LANA:} \\
% %   \vspace{-0.2cm}
%     \includegraphics[width=0.8\textwidth, trim={0cm 0 0cm 0cm},clip]{images/v2/efn_plot.pdf}
%   \\
%     \footnotesize{CPU optimized models:} \\
%     \resizebox{0.6\textwidth}{!}{%
%     \begin{tabular}{lclc}
%     \toprule
%     \multirow{2}{*}{Model} & Res. & Accuracy & Latency \\
%      & (px) & (\%) & Pytorch (ms) \\
%     \midrule
%     \midrule
%     EfficientNetB0          & 224  & 77.70 & 57\\
%     0.4xB2 (Xeon)           & 260 & 78.11 (+0.97) & 48 \\
%     0.5xB2 (Xeon)           & 260 & 78.87 (+1.17) & 58  \\
%     \midrule
%     EfficientNetB1          & 240 & 78.83 & 86\\
%     0.7xB2 (Xeon)           & 260 & 79.89 (+1.06) & 80 \\
%     \midrule
%     EfficientNetB2          & 260 & 80.07 & 113\\
%     \bottomrule
%     \end{tabular}
%     } 
%   \end{tabular}
%   \end{minipage}
%   \hfill

% \caption{Models optimized with LANA, evaluated on ImageNet-1K. Latency is computed for a batch of 128 images over 10 runs on actual hardware. Left: 3 families of models optimized for GPU. Right top: a visual summary of the table on the left, providing a detailed look at EfficientNets acceleration with LANA. Right bottom: EfficientNetV1 optimized for CPU inference.
% } 
% \label{tab:imagenet_comparison}
% \end{minipage}

%Accuracy dependency on compression ratio after the search and after finetuning.

==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/method_comparison.tex <==
% \begin{table*}[t]
% \scriptsize
% \centering
% \caption{Related method comparison. Time is mentioned in GPU hours by \texttt{h}, or ImageNet epochs by \texttt{e}. Our method assumes 197 candidate operations for the full pool, and only 2 (teacher and identity) for zero shot mode. \(L\) is the number of target architectures.} %otherwise pretraining cost increases linearly.}
% \label{tab:related_work}\vskip -5pt
% \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{l||c|c|c|c||c||c||c|c|c||c}
% \toprule
% Method & \multicolumn{4}{c||}{Knowledge Distillation} & Diverse & Design Space Size & Pretrain & Search & Train & Total  \\
%  & \multicolumn{4}{c||}{} & Operators &  & Cost & Cost & Cost & Cost  \\
% \hline
% & Layer & Block & Network & None &   & & \multicolumn{4}{c}{To Train \(L\) Architectures}\\
% \hline
% Once-For-All \cite{cai2020once} & & & & \checkmark & & \(> O\left(10^{19}\right)\) & 1205\texttt{e} & 40\texttt{h}& 75\texttt{e}$L$ & 75\texttt{e}\cdot(16+$L$)\\ 
% \hline
% AKD \cite{Liu_2020_CVPR} & & &\checkmark  & & \checkmark & \(> O\left(10^{13}\right)\) &
% 0 & 50000\texttt{e}\(L\) & 400\texttt{e}\(L\) & 50400\texttt{e}\(L\) \\ 
% %450\texttt{e}$N$ &  26\texttt{e}& 400\texttt{e}$N$ & 876\texttt{e}$N$ \\
% DNA \cite{Li_2020_CVPR} & &\checkmark & & &  & \(> O \left(10^{15}\right)\) & 320\texttt{e} & 14\texttt{h} & 450\texttt{e}$L$ & 320\texttt{e}\cdot(1+$1.4L$)\\

% DONNA \cite{moons2020distilling} & & \checkmark & & & \checkmark & \(> O\left(10^{13}\right)\) & 1920\texttt{e}\tablefootnote{can potentially be improved by parallelization} & 1500\texttt{e} + <1\texttt{h}$L$ & 50\texttt{e}$L$ & 50\texttt{e}\cdot(68+$L$) \\
% \hline
% This Work & \checkmark & & & & \checkmark & \(>O\left(10^{100}\right)\) & 197\texttt{e} & $<$1\texttt{h}$L$ & 100\texttt{e}$L$ &  100\texttt{e}\cdot(2+$L$)\\

% This Work - Zero shot& \checkmark & & & &  & \(>O\left(10^{2}\right)\) & 0 & $\sim$0 & 100\texttt{e}$L$ & 100\texttt{e}$L$\\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[t]
\scriptsize
\centering
\caption{Related method comparison. Time is mentioned in GPU hours by \texttt{h}, or ImageNet epochs by \texttt{e}. Our method assumes 197 candidate operations for the full pool, and only 2 (teacher and identity) for zero shot mode. \(L\) is the number of target architectures.} %otherwise pretraining cost increases linearly.}
\label{tab:related_work}\vskip -5pt
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l||c|c|c||c|c|c||c}
\toprule
Method & {Knowledge} & Diverse & Design Space & Pretrain & Search & Train & Total  \\
 & Distillation & Operators & Size & Cost & Cost & Cost & Cost  \\
\hline
&  &   & & \multicolumn{4}{c}{To Train \(L\) Architectures}\\
\hline
Once-For-All \cite{cai2020once} & None & & \(> O\left(10^{19}\right)\) & 1205\texttt{e} & 40\texttt{h}& 75\texttt{e}$L$ & 1205\texttt{e} + 75\texttt{e}$L$\\ 
\hline
AKD \cite{Liu_2020_CVPR} & Network & \checkmark & \(> O\left(10^{13}\right)\) &
0 & 50000\texttt{e}\(L\) & 400\texttt{e}\(L\) & 50400\texttt{e}\(L\) \\ 
%450\texttt{e}$N$ &  26\texttt{e}& 400\texttt{e}$N$ & 876\texttt{e}$N$ \\
DNA \cite{Li_2020_CVPR} & Block &  & \(> O \left(10^{15}\right)\) & 320\texttt{e} & 14\texttt{h}$L$ & 450\texttt{e}$L$ & 320\texttt{e} + 450\texttt{e}$L$\\
DONNA \cite{moons2020distilling} & Block & \checkmark & \(> O\left(10^{13}\right)\) & 1920\texttt{e}\tablefootnote{can potentially be improved by parallelization} & 1500\texttt{e} + <1\texttt{h}$L$ & 50\texttt{e}$L$ & 3420\texttt{e} + 50\texttt{e}$L$ \\
\hline
This Work & Layer & \checkmark & \(>O\left(10^{100}\right)\) & 197\texttt{e} & $<$1\texttt{h}$L$ & 100\texttt{e}$L$ &  197\texttt{e} + 100\texttt{e}$L$\\
This Work - Zero shot& None &  & \(>O\left(10^{2}\right)\) & 0 & $\sim$0 & 100\texttt{e}$L$ & 100\texttt{e}$L$\\
\bottomrule
\end{tabular}
}
\end{table*}



==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/nas_comparison.tex <==
% \begin{table}[t]
% \scriptsize
% \centering
% \vspace{-2mm}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccccc}
% \toprule
%                             & Only top-10 & Pretrained &   Finetuning  &  \multicolumn{2}{c}{Accuracy of 0.45xB2}   & Candidate    & Search \\
% Method                      & ops per cell&  weights   &during search  & No finetuning & Finetuning & evaluation & cost \\
% \midrule
% Integer optimization, top1  &             & \checkmark &            & 31.50            & 79.05 & -             & <1 CPU sec     \\
% Integer optimization, top50 &             & \checkmark &            & 39.03            & 79.17 & 0.15 GPU hour & 1.08 CPU min    \\
% Integer optimization, top100&             & \checkmark &            & 41.80            & 79.28 & 0.26 GPU hour & 4.5 CPU min    \\
% Integer optimization, top500&             & \checkmark &            & 46.36            & 79.54 & 1.5 GPU hour  & 6.8 CPU hours    \\
% Integer optimization, top1  & \checkmark  & \checkmark &            & 25.33            & 78.79 & -             & <1 CPU sec     \\  \hline
% Random, found 80 arch       & \checkmark  & \checkmark &            & 13.34            & 76.44 & 0.26 GPU hour & 1.4 min CPU    \\ \hline
% REINFORCE                   & \checkmark  &            & \checkmark & 0.88             & 69.93 &     -         & 16.3 GPU hours  \\
% REINFORCE                   & \checkmark  & \checkmark &            & 15.75            & 75.47 &    -          & 9.2  GPU hours  \\
% REINFORCE                   & \checkmark  & \checkmark & \checkmark & 7.61             & 74.20 &     -         & 16.3 GPU hours  \\ \hline
% Gumbel softmax              & \checkmark  &            & \checkmark & 0.83             & 65.19 &   -           & 61.6 GPU hours  \\ 
% Gumbel softmax              & \checkmark  & \checkmark &            & 21.27            & 75.61 &   -           & 58.3 GPU hours  \\
% Gumbel softmax              & \checkmark  & \checkmark & \checkmark & 24.97            & 78.85 &   -           & 61.6 GPU hours  \\ 
% \bottomrule
% \end{tabular}}
% \caption{Comparing methods for candidate selection (NAS). No finetuning accuracy is reported on 5\% of the training data after the search. Finetuned accruacy is reported for the entire validation set. 
% Full EfficientNet-B2 model training accuracy in the training mode is $77.88\%$ on 50 batches. 
% }
% \label{tab:ablation}
% % \vspace{-8mm}
% \end{table} 
% SNAS~\cite{xie2018snas} in this experiment; (iii) \textit{REINFORCE} is a stochastic optimization framework borrowed from reinforcement learning and adopted for architecture search~\cite{pham2018efficient, zoph2018learning,tan2019mnasnet}. We follow an E-NAS-like~\cite{pham2018efficient}
\begin{table}[t]

\centering
% \scriptsize
% \setlength{\tabcolsep}{3pt}
%\vspace{-0.3cm}
\caption{\small Comparing methods for candidate selection (NAS). Our proposed ILP is better ($+0.43\%$) and 821$\times$ faster.}
\label{tab:nas_comparison}
\vspace{-0.2cm}
\resizebox{0.35\textwidth}{!}{% % \vspace{-2mm}
\begin{tabular}{lcc}
\toprule
Method                            & Accuracy & Search cost\\
\midrule
\textbf{ILP, K=100 (ours)}                                            & 79.28   & 4.5 CPU/m \\
Random, found 80 arch                                  & 76.44   & 1.4 CPU/m     \\ 
SNAS~\citep{xie2018snas}                   &  74.20 & 16.3 GPU/h  \\ 
E-NAS~\citep{pham2018efficient}   &  78.85 & 61.6 GPU/h  \\ 
\bottomrule \vspace{-0.5cm}  
\end{tabular}
}
\end{table}



==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/only_skip.tex <==
\begin{table}
\centering
\caption{\small Zero-shot LANA with only skip connections. %Accuracy is reported after finetuning. 
\vspace{-0.2cm}} 
\label{tab:zero_shot_LANA}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Setup                            & \multicolumn{2}{c}{Top-1 Acc.} & Latency(ms) \\
                                 & Zero-shot &  All operations & TensorRT \\
\midrule
0.45xEfficientNetV1-B2            & 78.68 & 79.71   & 16.2\\
0.55xEfficientNetV1-B2            & 79.40 & 80.11   & 20.6\\
\midrule
EfficientNetV1-B0         & \multicolumn{2}{c}{77.70} & 17.9 \\
EfficientNetV1-B2            & \multicolumn{2}{c}{80.07} & 38.8\\
\bottomrule 
\end{tabular}
}
\end{table}


==> LANA_CVPR2022_arxiv%20(Version%20281)/tables/search_space.tex <==
\begin{table}
    \centering
    \setlength{\tabcolsep}{3pt}


\caption{Impact of the search space on 0.55$\times$EfficientNetV1-B2 compression. Two operations correspond to Zero-shot LANA.}
\label{tab:search_space}
    \vspace{-0.2cm}
\resizebox{0.39\textwidth}{!}{%
\begin{tabular}{lx{0.07\textwidth}x{0.08\textwidth}x{0.08\textwidth}x{0.08\textwidth}}
\toprule
% \multicolumn{4}{c}{Number of operations per layer} \\ 
Operations \# & 2 & 5 & 10 & All \\
\midrule
Space size   & $O(10^{7})$ &  $O(10^{16})$ & $O(10^{23})$ & $O(10^{46})$ \\
Accuracy  & 79.40 &	79.52 &	79.66 &	80.00 \\

\bottomrule

% \bottomrule
\end{tabular}}
\end{table}


==> LANA_CVPR2022_arxiv%20(Version%20281)/tikzfigures/method_figure_arrows.tex <==
\tikzstyle{teachernode} = [rectangle, rounded corners, text centered, draw=black, fill=green!20]
\tikzstyle{studentnode} = [rectangle, rounded corners, text centered, draw=black, fill=red!20]
\tikzstyle{dotsnode} = [rectangle, rounded corners, draw=white, fill=white!20]
\tikzstyle{infarrow} = [thick, ->, >=stealth]
\tikzstyle{distilarrow} = [thick, ->, >=stealth, dashed]
%\begin{minipage}{.4\textwidth}
%\tikzstyle{teachernode} = [rectangle, rounded corners, text centered, draw=black, fill=green!20]
%\tikzstyle{studentnode} = [rectangle, rounded corners, text centered, draw=black, fill=red!20]
%\tikzstyle{dotsnode} = [rectangle, rounded corners, draw=white, fill=white!20]
%\tikzstyle{infarrow} = [thick, ->, >=stealth]
%\tikzstyle{distilarrow} = [thick, ->, >=stealth, dashed]

%\begin{figure}
%\subfigure[Before]
%{
\begin{figure}[h!]
\begin{subfigure}{.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{0}\)};
\node (teacherd) [dotsnode, below of=teacher1] {\(\vdots\)};
\node (teachern) [teachernode, below of=teacherd] {\(o_{n}\)};
\node (pool) [teachernode, below of=teachern] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (dotsd0) [dotsnode, right of=teacherd, yshift=-0.3cm] {\(\vdots\)};
\node (dotsd1) [dotsnode, right of=dotsd0] {\(\vdots\)};
\node (dotsdd) [dotsnode, right of=dotsd1] {\(\ddots\)};
\node (dotsdn) [dotsnode, right of=dotsdd] {\(\vdots\)};
\node (studentn0) [studentnode, right of=teachern, yshift=-0.5cm] {\(s_{n0}\)};
\node (studentn1) [studentnode, right of=studentn0] {\(s_{n1}\)};
\node (dotsnn) [dotsnode, right of=studentn1] {\(\cdots\)};
\node (studentnn) [studentnode, right of=dotsnn] {\(s_{nn}\)};
\draw [infarrow] (stem) -- (teacher0);
\draw [distilarrow] (teacher0) -| (student00);
\draw [distilarrow] (teacher0) -| (student01);
\draw [distilarrow] (teacher0) -| (student0n);
\draw [infarrow] (teacher0) -- (teacher1);
\draw [distilarrow] (teacher1) -| (student10);
\draw [distilarrow] (teacher1) -| (student11);
\draw [distilarrow] (teacher1) -| (student1n);
\draw [infarrow] (teacher1) -- (teacherd);
\draw [infarrow] (teacherd) -- (teachern);
\draw [distilarrow] (teachern) -| (studentn0);
\draw [distilarrow] (teachern) -| (studentn1);
\draw [distilarrow] (teachern) -| (studentnn);
\draw [infarrow] (teachern) -- (pool);
\draw [infarrow] (pool) -- (fc);
\end{tikzpicture}
\caption{Pretraining}
\end{subfigure}\hspace{0.1\textwidth}
%}
%\end{figure}
%\end{minipage}
%\begin{minipage}{0.2\textwidth}
\begin{subfigure}{0.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed][scale=0.33]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{0}\)};
\node (teacherd) [dotsnode, below of=teacher1] {\(\vdots\)};
\node (teachern) [teachernode, below of=teacherd] {\(o_{n}\)};
\node (pool) [teachernode, below of=teachern] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (dotsd0) [dotsnode, right of=teacherd, yshift=-0.3cm] {\(\vdots\)};
\node (dotsd1) [dotsnode, right of=dotsd0] {\(\vdots\)};
\node (dotsdd) [dotsnode, right of=dotsd1] {\(\ddots\)};
\node (dotsdn) [dotsnode, right of=dotsdd] {\(\vdots\)};
\node (studentn0) [studentnode, right of=teachern, yshift=-0.5cm] {\(s_{n0}\)};
\node (studentn1) [studentnode, right of=studentn0] {\(s_{n1}\)};
\node (dotsnn) [dotsnode, right of=studentn1] {\(\cdots\)};
\node (studentnn) [studentnode, right of=dotsnn] {\(s_{nn}\)};
%\draw [infarrow] (stem) -- (teacher0);
%\draw [distilarrow] (teacher0) -| (student00);
%\draw [distilarrow] (teacher0) -| (student01);
%\draw [distilarrow] (teacher0) -| (student0n);
%\draw [infarrow] (teacher0) -- (teacher1);
%\draw [distilarrow] (teacher1) -| (student10);
%\draw [distilarrow] (teacher1) -| (student11);
%\draw [distilarrow] (teacher1) -| (student1n);
%\draw [infarrow] (teacher1) -- (teacherd);
%\draw [infarrow] (teacherd) -- (teachern);
%\draw [distilarrow] (teachern) -| (studentn0);
%\draw [distilarrow] (teachern) -| (studentn1);
%\draw [distilarrow] (teachern) -| (studentnn);
%\draw [infarrow] (teachern) -- (pool);
\draw [infarrow] (stem) -- (student01);
\draw [infarrow] (student01) -- (student10);
\draw [infarrow] (student10) -- (dotsdn);
\draw [infarrow] (dotsd0) -- (teachern);
\draw [infarrow] (teachern) -- (pool);
\draw [infarrow] (pool) -- (fc);
\end{tikzpicture}
\caption{Search}
\end{subfigure}
\end{figure}
%\end{minipage}

==> LANA_CVPR2022_arxiv%20(Version%20281)/tikzfigures/method_figure_three_layers.tex <==
\tikzstyle{teachernode} = [rectangle, rounded corners, text centered, draw=black, fill=green!20]
\tikzstyle{studentnode} = [rectangle, rounded corners, text centered, draw=black, fill=red!20]
\tikzstyle{dotsnode} = [rectangle, rounded corners, draw=white, fill=white!20]
\tikzstyle{infarrow} = [thick, ->, >=stealth]
\tikzstyle{distilarrow} = [thick, ->, >=stealth, dashed]

\begin{figure}[h!]
\begin{subfigure}{.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{1}\)};
\node (teacher2) [teachernode, below of=teacher1] {\(o_{2}\)};
\node (pool) [teachernode, below of=teacher2] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (student20) [studentnode, right of=teacher2, yshift=-0.5cm] {\(s_{20}\)};
\node (student21) [studentnode, right of=student20] {\(s_{21}\)};
\node (dots2n) [dotsnode, right of=student21] {\(\cdots\)};
\node (student2n) [studentnode, right of=dots2n] {\(s_{2n}\)};
\draw [infarrow] (stem) -- (teacher0);
\draw [distilarrow] (teacher0) -| (student00);
\draw [distilarrow] (teacher0) -| (student01);
\draw [distilarrow] (teacher0) -| (student0n);
\draw [infarrow] (teacher0) -- (teacher1);
\draw [distilarrow] (teacher1) -| (student10);
\draw [distilarrow] (teacher1) -| (student11);
\draw [distilarrow] (teacher1) -| (student1n);
\draw [infarrow] (teacher1) -- (teacher2);
\draw [distilarrow] (teacher2) -| (student20);
\draw [distilarrow] (teacher2) -| (student21);
\draw [distilarrow] (teacher2) -| (student2n);
\draw [infarrow] (teacher2) -- (pool);
\draw [infarrow] (pool) -- (fc);
\end{tikzpicture}
\caption{Pretraining}
\end{subfigure}\hspace{0.1\textwidth}
%
\begin{subfigure}{0.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed][scale=0.33]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{1}\)};
\node (teacher2) [teachernode, below of=teacher1] {\(o_{2}\)};
\node (pool) [teachernode, below of=teacher2] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (student20) [studentnode, right of=teacher2, yshift=-0.5cm] {\(s_{20}\)};
\node (student21) [studentnode, right of=student20] {\(s_{21}\)};
\node (dots2n) [dotsnode, right of=student21] {\(\cdots\)};
\node (student2n) [studentnode, right of=dots2n] {\(s_{2n}\)};
\draw [infarrow] (stem) -- (student01);
\draw [infarrow] (student01) -- (student10);
\draw [infarrow] (student10) -- (teacher2);
\draw [infarrow] (teacher2) -- (pool);
\draw [infarrow] (pool) -- (fc);

\end{tikzpicture}
\caption{Search}
\end{subfigure}
\label{fig:method}
\end{figure}

==> LANA_CVPR2022_arxiv%20(Version%20281)/tikzfigures/method_no_offsets.tex <==
\tikzstyle{teachernode} = [rectangle, rounded corners, text centered, draw=black, fill=green!20]
\tikzstyle{studentnode} = [rectangle, rounded corners, text centered, draw=black, fill=red!20]
\tikzstyle{dotsnode} = [rectangle, rounded corners, draw=white, fill=white!20]
\tikzstyle{infarrow} = [thick, ->, >=stealth]
\tikzstyle{distilarrow} = [thick, ->, >=stealth, dashed]

\begin{figure}[h!]
\begin{subfigure}{.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{1}\)};
\node (teacher2) [teachernode, below of=teacher1] {\(o_{2}\)};
\node (pool) [teachernode, below of=teacher2] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (student20) [studentnode, right of=teacher2, yshift=-0.5cm] {\(s_{20}\)};
\node (student21) [studentnode, right of=student20] {\(s_{21}\)};
\node (dots2n) [dotsnode, right of=student21] {\(\cdots\)};
\node (student2n) [studentnode, right of=dots2n] {\(s_{2n}\)};
\draw [infarrow] (stem) -- (teacher0);
\draw [distilarrow] (teacher0) -| (student00);
\draw [distilarrow] (teacher0) -| (student01);
\draw [distilarrow] (teacher0) -| (student0n);
\draw [infarrow] (teacher0) -- (teacher1);
\draw [distilarrow] (teacher1) -| (student10);
\draw [distilarrow] (teacher1) -| (student11);
\draw [distilarrow] (teacher1) -| (student1n);
\draw [infarrow] (teacher1) -- (teacher2);
\draw [distilarrow] (teacher2) -| (student20);
\draw [distilarrow] (teacher2) -| (student21);
\draw [distilarrow] (teacher2) -| (student2n);
\draw [infarrow] (teacher2) -- (pool);
\draw [infarrow] (pool) -- (fc);
\end{tikzpicture}
\caption{Pretraining}
\end{subfigure}\hspace{0.1\textwidth}
%
\begin{subfigure}{0.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed][scale=0.33]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{1}\)};
\node (teacher2) [teachernode, below of=teacher1] {\(o_{2}\)};
\node (pool) [teachernode, below of=teacher2] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (student20) [studentnode, right of=teacher2, yshift=-0.5cm] {\(s_{20}\)};
\node (student21) [studentnode, right of=student20] {\(s_{21}\)};
\node (dots2n) [dotsnode, right of=student21] {\(\cdots\)};
\node (student2n) [studentnode, right of=dots2n] {\(s_{2n}\)};
\draw [infarrow] (stem) -- (student01);
\draw [infarrow] (student01) -- (student10);
\draw [infarrow] (student10) -- (teacher2);
\draw [infarrow] (teacher2) -- (pool);
\draw [infarrow] (pool) -- (fc);

\end{tikzpicture}
\caption{Search}
\end{subfigure}
\end{figure}

==> broader_impact.tex <==

\subsection{Analysis}

\input{tables/cpu_restable_wrap}
All studies in this section are performed with the setting of compressing  EfficientNet-B2 by $0.45\times$ to match the latency of B0. Finetuning is reduced to 50 epochs only, while search is limited to 50 architectures. Additional ablation studies on the length of pretraining, contribution of distillation loss for finetuning, and importance of pre-loading weights can be found in Appendix.

\textbf{Pretraining Stage.}
To gain more insights into the tradeoff between the accuracy and speed of each operation, we analyze the the pretrained candidate operation pool. Figure~\ref{fig:phase2} highlights tradeoff for three layers spaced equally throughout the network. In general,
we observe that no operation outperforms the teacher in terms of accuracy.
We also see that it is increasingly difficult to recover the teacher's accuracy as the depth in the network increases. For example, the best operation at layer 7 can recover around 100\% of the teacher's performance, whereas it drops to 99\% by layer 21. The speedups achievable are roughly comparable across different depths, however we note that achieving such speedups earlier in the network is particularly effective towards reducing total latency due to the first third of the layers accounting for 54\% of the total inference time. 

Looking at individual operations, we observe that inverted residual blocks (\texttt{efn}, \texttt{efnv2}) are the most accurate throughout the network, at the expense of increased computational cost (\emph{i.e.,} lower speedups). Dense convolutions (\texttt{cb\_stack}, \texttt{cb\_bottle}, \texttt{conv\_cs}, \texttt{cb\_res}) exhibit a good compromise between accuracy and speed, with stacked convolutions being particularly effective earlier in the network (\emph{e.g.,} see 7$^\text{th}$ layer). The identity operation unsurprisingly achieves very high speedups at the expense of increasingly poor accuracy compared to the teacher as a function of depth. Visual transformer blocks (\texttt{ViT}) and bottleneck transformer blocks (\texttt{bot\_trans}) show neither a speedup advantage nor are able to recover the accuracy of the teacher. Indeed, their performance, across all axes, gets progressively worse as a function of depth, and as a result they are never selected during the search.



\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth,trim=.25cm .25cm .25cm .25cm,clip=true]{images/pretraining_efnb2_3layers.pdf}
    \caption{Result of the pretraining stage for EfficientNetB2, showing three layers equally spaced throughout the network: 7, 14 and 21. Speedup is measured as the ratio between the latency of the teacher and the latency of the student operation (higher is better). We measure latency using Pytorch FP16. Accuracy is the ratio of the operation's accuracy and the teacher's (higher is better). The dashed black lines correspond to the teacher.} 
    \label{fig:phase2}
\end{figure}

\textbf{Architecture Search.}
We compare our implementation of architecture search with other popular approaches to solve Eq.~(\ref{eq:nas_formulation}), including: (i) \textit{Random} architecture sampling within a latency constrain; (ii) \textit{Differentiable search with Gumbel Softmax} -- a popular approach in NAS to relax binary optimization as a continuous variable optimization via learning the sampling the distribution~\cite{xie2018snas, Wu_2019_CVPR,vahdat2020unas}. We follow SNAS~\cite{xie2018snas} in this experiment; (iii) \textit{REINFORCE} is a stochastic optimization framework borrowed from reinforcement learning and adopted for architecture search~\cite{pham2018efficient, zoph2018learning,tan2019mnasnet}. We follow an E-NAS-like~\cite{pham2018efficient} architecture search. Both learning-based solutions (ii) and (iii) benefit from simultaneous architecture and weight tuning, therefore we do search with and without those updates. Since both Gumbel Softmax and REINFORCE are compute and memory intensive, we only use the top 10 operations per layer, chosen based on high accuracy and low latency. 

Different variations of NAS are compared in Table~\ref{tab:ablation}. We make the following observations: (i) the proposed integer optimization for search significantly outperforms Gumbel Softmax and REINFORCE while being orders of magnitude faster in search; (ii) Both Gumbel Softmax and REINFORCE perform poorly when weights are not initialized using our pretraining phase, emphasizing on the importance of phase one. (iii) The substantial improvement is obtained with increasing number of candidate operations for integer optimization while Gumbel Softmax and REINFORCE cannot handle large number of operations; (iv) there is a strong correlation between the loss after search on training set with the final one on the validation set; (v) the search and evaluation costs are significantly lower for integer optimization; (vi) final accuracy increases with increasing the number of candidate architectures $k$ for linear optimization. Accuracy correlation before and after search allows us to evaluate candidates without training candidate architectures, performing search at minimal cost. 

\input{tables/nas_comparison.tex}


\textbf{Common Operations.} In Appendix, we analyse the distribution of the selected operations by solving for 100 architecture candidates with Eq.~\ref{eq:integer} and picking the top-10 of them. We observe the following insights: (i) teacher operations are selected most frequently, it is expected as we only transform the model and no operations can beat teacher in terms of accuracy; 
(ii) identity operation is selected more often for architectures with higher compression rates versus small compression;
(iii) dense convolution blocks tend to appear more for larger models like EfficientNet-B6 to speed them up. 


\textbf{Final Architectures.} We analyze final architectures (detailed structures in Appendix) and observe: (i) Teacher's operations are usually selected in the tail of the network as they are relatively fast and approximating them results in the highest error. (ii) Teacher operation is preferred for downsampling layers (e.g. stride is 2). Those cells are hard to approximate as well. (iii) Transformer blocks are never selected, probably because they 
require significantly longer pretraining on larger datasets. (iv) As the networks get larger, we see more dense convolutions being selected rather than depth-wise separable counterparts. (v) Identity operations are more often seen in the first half of the network for architectures when we want to achieve high compression. 


\begin{wrapfigure}{r}{0.35\textwidth}
    \vspace{-0.5cm}
    \includegraphics[width=0.99\textwidth, trim={0.25cm 0.25cm 0.25cm 0.25cm},clip]{images/compression_vs_final_acc.pdf}
    \vspace{-0.7cm}
    \caption{\small Accuracy vs. compression}
    % \vspace{-0.65cm}
    \label{fig:train_vs_va}
\end{wrapfigure}

\textbf{Compression / Accuracy Trade-off.} Compressing any given network with different rates will produce a family of accelerated networks. However, accuracy will starts decreasing with aggressive compression rates. We demonstrate this effect in Figure~\ref{fig:train_vs_va}, where we see a sharp drop in accuracy with compression rates below $0.3$. It can be explained by a weak prior on accuracy used in our linear optimization to characterize non-linear dynamics of networks, which in turn makes our relaxation a poor approximation of the actual loss.

==> final_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}
% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See the \textbf{Limitation} section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We included detailed discussions on the associated computation in GPU hours as required by HANT. We also include additional discussion in the \textbf{Broader Impact} section.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA
	\item Did you include complete proofs of all theoretical results?
    \answerNA
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include code and HANT-based ImageNet EfficientNet Derivatives in supplemental materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Sec.~\ref{sec:experiments}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We did not repeat NAS runs amid high GPU computation requirement when combining both phases in overall pipeline. We report error bars for latency measurements.} \DY{PLEASE CHECK - UPDATE after experiments.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We included detailed descriptions of each computation environment alongside our experiments.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets... 
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite relevant creators/datasets in both the main paper and the Appendix.} 
  \item Did you mention the license of the assets?
    \answerYes{We mention the license of the assets in Appendix.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We used publicly available assets and did not introduce new ones.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{All datasets we used are publicly available and we specified the dataset names in experiments.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects in this paper.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects in this paper.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects in this paper.}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> images/imagenet_gpu.tex <==
\begin{figure}[t]
     \centering
     \includegraphics[width=0.45\textwidth, trim={0cm 0 0cm 0cm},clip]{images/v2/efn_plot.pdf}
     \caption{A visual summary of the EfficientNetV1 and EfficientNetV2 model families accelerated by LANA. Accelerated EfficientNetV1 models outperform EfficientNetV2 models.}
     \label{fig:imagenet_comparison}
 \end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/candidate_evaluation.tex <==
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\vspace{0cm}
\vspace{0mm}
\caption{\small Candidate evaluation metrics for model ranking before and after finetuning. \vspace{-0.0cm}} \label{tab:candidate_evaluation_metrics}
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Correlation & Accuracy & Cross-entropy & KL divergence & MSE \\
\midrule
Kendal Tau  & 0.835 & 0.824 & 0.832 & 0.811 \\
Spearman    & 0.945 & 0.947 & 0.954 & 0.944\\ 
\bottomrule \vspace{-0.0cm}
\end{tabular}
}
% \vspace{-8mm}
\end{table}
%\vspace{-0.3cm}

% kdt, 0.772, spearman, 0.914
% metric:  eval_loss
% kdt, 0.776, spearman, 0.924
% metric:  eval_kdloss
% kdt, 0.673, spearman, 0.843
% metric:  eval_mseloss
% kdt, 0.475, spearman, 0.647

% metric:  train_accuracy
% kdt, 0.835, spearman, 0.945
% metric:  train_loss
% kdt, 0.824, spearman, 0.947
% metric:  train_kdloss
% kdt, 0.832, spearman, 0.954
% metric:  train_mseloss
% kdt, 0.811, spearman, 0.944

==> tables/gpu_results.tex <==
    \begin{table}[h]
    \centering
    \caption{CPU optimized models:} 
    \label{tab:cpu_results}
    \resizebox{0.4\textwidth}{!}{%
    
    \begin{tabular}{lclc}
    \toprule
    \multirow{2}{*}{Model} & Res. & Accuracy & Latency \\
     & (px) & (\%) & Pytorch (s) \\
    \midrule
    \midrule
    EfficientNetB0          & 224  & 77.70 & 0.057 $\pm$ 0.001  \\
    0.4xB2 (Xeon)           & 260 & 78.11 (+0.97) & 0.048 $\pm$ 0.001 \\
    0.5xB2 (Xeon)           & 260 & 78.87 (+1.17) & 0.058 $\pm$ 0.001 \\
    \midrule
    EfficientNetB1          & 240 & 78.83 & 0.086 $\pm$ 0.001 \\
    0.7xB2 (Xeon)           & 260 & 79.89 (+1.06) & 0.080 $\pm$ 0.001 \\
    \midrule
    EfficientNetB2          & 260 & 80.39 & 0.113 $\pm$ 0.002 \\
    \bottomrule
    \end{tabular}
    }
    \end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth, trim={0cm 0 1cm 1cm},clip]{images/v2/effnv2.pdf}
    \caption{EfficientNets compression with HANT for V100 GPU:}
    \label{fig:result_efn_plot}
\end{figure}

\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.4\textwidth}{!}{%
    \begin{tabular}{lclcc}
    \toprule
    \multirow{2}{*}{Model} & Res & Accuracy & \multicolumn{2}{c}{Latency(ms) per 128 images} \\
     & {px} & (\%)  & TensorRT & PyTorch\\
    \midrule
    \midrule
    \multicolumn{5}{c}{\textbf{EfficientNetV1}}  \\
    \midrule
    \midrule
    EfficientNetV1-B0         & 224  & 77.70 & 17.9 & 35.6 \\
    0.45xB2                & 260  & \textbf{79.71 (+2.01)} & \textbf{16.2} & 30.2\\      
    \midrule
    EfficientNetV1-B1         & 240  & 78.83 & 29.3 & 59.0 \\
    0.55xB2                & 260  & 80.11 (+1.28) & \textbf{20.6} & 48.7\\      
    0.2xB4                 & 380  & 80.33 (+1.50) & 33.0 & 64.5\\
    0.25xB4                 & 380  & \textbf{81.83 (+3.00)} & 30.4 & 64.5\\
    \midrule
    EfficientNetV1-B2         & 260  & 80.39 & 38.2 & 77.1 \\
    0.3xB4                 & 380  & \textbf{82.16 (+1.77)} & \textbf{38.8} & 81.8\\        
    \midrule
    EfficientNetV1-B3         & 300  & 81.67 & 67.2 & 125.9 \\
    0.5xB4                 & 380  & \textbf{82.66 (+0.99)} & \textbf{61.4} & 0.1914\\            
    \midrule
    EfficientNetV1-B4         & 380  & 83.02 & 132.0 & ?  \\
    % 0.2xB6               & 528  & 82.57 & \textbf{0.1515} & 0.3243 & 0.5654 \\
    0.25xB6                & 528  & \textbf{83.77 (+0.75)} &  \textbf{128.8} & ?\\
    \midrule
    EfficientNetV1-B5         & 456  & 83.81 & 265.7 & ?  \\
    % 0.45xB6                & 528  & \textbf{83.85 (+0.04)} & \textbf{0.3560} & 0.7261\\
    0.5xB6                 & 528  & \textbf{83.99 (+0.18)} & \textbf{266.5} & ? \\
    \midrule
    EfficientNetV1-B6         & 528  & 84.11 & 466.7 & ?  \\
        \midrule
    \midrule
    \multicolumn{5}{c}{\textbf{EfficientNetV2}}  \\
    \midrule
    \midrule
    EfficientNetV2-B1         & 240  & 79.46 & 17.9 & 44.7 \\
    0.45xB3                   & 300  & \textbf{80.30 (+0.84)} & \textbf{17.8} & 43.0\\      
    \midrule
    EfficientNetV2-B2         & 260  & 80.21 & 24.3 & 58.9 \\
    0.6xB3                    & 300  & \textbf{81.14 (+0.93)} & \textbf{23.8} & 56.1\\      
    \midrule
    EfficientNetV2-B3       & 300  & 81.97 & 41.2 & 91.6 \\
    \midrule
    \midrule
    \multicolumn{5}{c}{\textbf{ResNeST50d\_1s4x24d}}  \\
    \midrule
    \midrule
    ResNeST50       & 224  & 80.99 & 32.3 & 74.0 \\
    0.7x            & 224  & 80.85 & \textbf{22.3(1.45x)} & 52.7 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Models optimized for GPU inference}
    \label{tab:gpu_results}
\end{table}


==> tikzfigures/method_figure_arrows.tex <==
\tikzstyle{teachernode} = [rectangle, rounded corners, text centered, draw=black, fill=green!20]
\tikzstyle{studentnode} = [rectangle, rounded corners, text centered, draw=black, fill=red!20]
\tikzstyle{dotsnode} = [rectangle, rounded corners, draw=white, fill=white!20]
\tikzstyle{infarrow} = [thick, ->, >=stealth]
\tikzstyle{distilarrow} = [thick, ->, >=stealth, dashed]
%\begin{minipage}{.4\textwidth}
%\tikzstyle{teachernode} = [rectangle, rounded corners, text centered, draw=black, fill=green!20]
%\tikzstyle{studentnode} = [rectangle, rounded corners, text centered, draw=black, fill=red!20]
%\tikzstyle{dotsnode} = [rectangle, rounded corners, draw=white, fill=white!20]
%\tikzstyle{infarrow} = [thick, ->, >=stealth]
%\tikzstyle{distilarrow} = [thick, ->, >=stealth, dashed]

%\begin{figure}
%\subfigure[Before]
%{
\begin{figure}[h!]
\begin{subfigure}{.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{0}\)};
\node (teacherd) [dotsnode, below of=teacher1] {\(\vdots\)};
\node (teachern) [teachernode, below of=teacherd] {\(o_{n}\)};
\node (pool) [teachernode, below of=teachern] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (dotsd0) [dotsnode, right of=teacherd, yshift=-0.3cm] {\(\vdots\)};
\node (dotsd1) [dotsnode, right of=dotsd0] {\(\vdots\)};
\node (dotsdd) [dotsnode, right of=dotsd1] {\(\ddots\)};
\node (dotsdn) [dotsnode, right of=dotsdd] {\(\vdots\)};
\node (studentn0) [studentnode, right of=teachern, yshift=-0.5cm] {\(s_{n0}\)};
\node (studentn1) [studentnode, right of=studentn0] {\(s_{n1}\)};
\node (dotsnn) [dotsnode, right of=studentn1] {\(\cdots\)};
\node (studentnn) [studentnode, right of=dotsnn] {\(s_{nn}\)};
\draw [infarrow] (stem) -- (teacher0);
\draw [distilarrow] (teacher0) -| (student00);
\draw [distilarrow] (teacher0) -| (student01);
\draw [distilarrow] (teacher0) -| (student0n);
\draw [infarrow] (teacher0) -- (teacher1);
\draw [distilarrow] (teacher1) -| (student10);
\draw [distilarrow] (teacher1) -| (student11);
\draw [distilarrow] (teacher1) -| (student1n);
\draw [infarrow] (teacher1) -- (teacherd);
\draw [infarrow] (teacherd) -- (teachern);
\draw [distilarrow] (teachern) -| (studentn0);
\draw [distilarrow] (teachern) -| (studentn1);
\draw [distilarrow] (teachern) -| (studentnn);
\draw [infarrow] (teachern) -- (pool);
\draw [infarrow] (pool) -- (fc);
\end{tikzpicture}
\caption{Pretraining}
\end{subfigure}\hspace{0.1\textwidth}
%}
%\end{figure}
%\end{minipage}
%\begin{minipage}{0.2\textwidth}
\begin{subfigure}{0.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed][scale=0.33]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{0}\)};
\node (teacherd) [dotsnode, below of=teacher1] {\(\vdots\)};
\node (teachern) [teachernode, below of=teacherd] {\(o_{n}\)};
\node (pool) [teachernode, below of=teachern] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (dotsd0) [dotsnode, right of=teacherd, yshift=-0.3cm] {\(\vdots\)};
\node (dotsd1) [dotsnode, right of=dotsd0] {\(\vdots\)};
\node (dotsdd) [dotsnode, right of=dotsd1] {\(\ddots\)};
\node (dotsdn) [dotsnode, right of=dotsdd] {\(\vdots\)};
\node (studentn0) [studentnode, right of=teachern, yshift=-0.5cm] {\(s_{n0}\)};
\node (studentn1) [studentnode, right of=studentn0] {\(s_{n1}\)};
\node (dotsnn) [dotsnode, right of=studentn1] {\(\cdots\)};
\node (studentnn) [studentnode, right of=dotsnn] {\(s_{nn}\)};
%\draw [infarrow] (stem) -- (teacher0);
%\draw [distilarrow] (teacher0) -| (student00);
%\draw [distilarrow] (teacher0) -| (student01);
%\draw [distilarrow] (teacher0) -| (student0n);
%\draw [infarrow] (teacher0) -- (teacher1);
%\draw [distilarrow] (teacher1) -| (student10);
%\draw [distilarrow] (teacher1) -| (student11);
%\draw [distilarrow] (teacher1) -| (student1n);
%\draw [infarrow] (teacher1) -- (teacherd);
%\draw [infarrow] (teacherd) -- (teachern);
%\draw [distilarrow] (teachern) -| (studentn0);
%\draw [distilarrow] (teachern) -| (studentn1);
%\draw [distilarrow] (teachern) -| (studentnn);
%\draw [infarrow] (teachern) -- (pool);
\draw [infarrow] (stem) -- (student01);
\draw [infarrow] (student01) -- (student10);
\draw [infarrow] (student10) -- (dotsdn);
\draw [infarrow] (dotsd0) -- (teachern);
\draw [infarrow] (teachern) -- (pool);
\draw [infarrow] (pool) -- (fc);
\end{tikzpicture}
\caption{Search}
\end{subfigure}
\end{figure}
%\end{minipage}

==> tikzfigures/method_figure_three_layers.tex <==
\tikzstyle{teachernode} = [rectangle, rounded corners, text centered, draw=black, fill=green!20]
\tikzstyle{studentnode} = [rectangle, rounded corners, text centered, draw=black, fill=red!20]
\tikzstyle{dotsnode} = [rectangle, rounded corners, draw=white, fill=white!20]
\tikzstyle{infarrow} = [thick, ->, >=stealth]
\tikzstyle{distilarrow} = [thick, ->, >=stealth, dashed]

\begin{figure}[h!]
\begin{subfigure}{.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{1}\)};
\node (teacher2) [teachernode, below of=teacher1] {\(o_{2}\)};
\node (pool) [teachernode, below of=teacher2] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (student20) [studentnode, right of=teacher2, yshift=-0.5cm] {\(s_{20}\)};
\node (student21) [studentnode, right of=student20] {\(s_{21}\)};
\node (dots2n) [dotsnode, right of=student21] {\(\cdots\)};
\node (student2n) [studentnode, right of=dots2n] {\(s_{2n}\)};
\draw [infarrow] (stem) -- (teacher0);
\draw [distilarrow] (teacher0) -| (student00);
\draw [distilarrow] (teacher0) -| (student01);
\draw [distilarrow] (teacher0) -| (student0n);
\draw [infarrow] (teacher0) -- (teacher1);
\draw [distilarrow] (teacher1) -| (student10);
\draw [distilarrow] (teacher1) -| (student11);
\draw [distilarrow] (teacher1) -| (student1n);
\draw [infarrow] (teacher1) -- (teacher2);
\draw [distilarrow] (teacher2) -| (student20);
\draw [distilarrow] (teacher2) -| (student21);
\draw [distilarrow] (teacher2) -| (student2n);
\draw [infarrow] (teacher2) -- (pool);
\draw [infarrow] (pool) -- (fc);
\end{tikzpicture}
\caption{Pretraining}
\end{subfigure}\hspace{0.1\textwidth}
%
\begin{subfigure}{0.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed][scale=0.33]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{1}\)};
\node (teacher2) [teachernode, below of=teacher1] {\(o_{2}\)};
\node (pool) [teachernode, below of=teacher2] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (student20) [studentnode, right of=teacher2, yshift=-0.5cm] {\(s_{20}\)};
\node (student21) [studentnode, right of=student20] {\(s_{21}\)};
\node (dots2n) [dotsnode, right of=student21] {\(\cdots\)};
\node (student2n) [studentnode, right of=dots2n] {\(s_{2n}\)};
\draw [infarrow] (stem) -- (student01);
\draw [infarrow] (student01) -- (student10);
\draw [infarrow] (student10) -- (teacher2);
\draw [infarrow] (teacher2) -- (pool);
\draw [infarrow] (pool) -- (fc);

\end{tikzpicture}
\caption{Search}
\end{subfigure}
\label{fig:method}
\end{figure}

==> tikzfigures/method_no_offsets.tex <==
\tikzstyle{teachernode} = [rectangle, rounded corners, text centered, draw=black, fill=green!20]
\tikzstyle{studentnode} = [rectangle, rounded corners, text centered, draw=black, fill=red!20]
\tikzstyle{dotsnode} = [rectangle, rounded corners, draw=white, fill=white!20]
\tikzstyle{infarrow} = [thick, ->, >=stealth]
\tikzstyle{distilarrow} = [thick, ->, >=stealth, dashed]

\begin{figure}[h!]
\begin{subfigure}{.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{1}\)};
\node (teacher2) [teachernode, below of=teacher1] {\(o_{2}\)};
\node (pool) [teachernode, below of=teacher2] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (student20) [studentnode, right of=teacher2, yshift=-0.5cm] {\(s_{20}\)};
\node (student21) [studentnode, right of=student20] {\(s_{21}\)};
\node (dots2n) [dotsnode, right of=student21] {\(\cdots\)};
\node (student2n) [studentnode, right of=dots2n] {\(s_{2n}\)};
\draw [infarrow] (stem) -- (teacher0);
\draw [distilarrow] (teacher0) -| (student00);
\draw [distilarrow] (teacher0) -| (student01);
\draw [distilarrow] (teacher0) -| (student0n);
\draw [infarrow] (teacher0) -- (teacher1);
\draw [distilarrow] (teacher1) -| (student10);
\draw [distilarrow] (teacher1) -| (student11);
\draw [distilarrow] (teacher1) -| (student1n);
\draw [infarrow] (teacher1) -- (teacher2);
\draw [distilarrow] (teacher2) -| (student20);
\draw [distilarrow] (teacher2) -| (student21);
\draw [distilarrow] (teacher2) -| (student2n);
\draw [infarrow] (teacher2) -- (pool);
\draw [infarrow] (pool) -- (fc);
\end{tikzpicture}
\caption{Pretraining}
\end{subfigure}\hspace{0.1\textwidth}
%
\begin{subfigure}{0.33\textwidth}
\begin{tikzpicture}[node distance=1cm, framed][scale=0.33]
\node (stem) [teachernode] {stem};
\node (teacher0) [teachernode, below of=stem] {\(o_{0}\)};
\node (teacher1) [teachernode, below of=teacher0] {\(o_{1}\)};
\node (teacher2) [teachernode, below of=teacher1] {\(o_{2}\)};
\node (pool) [teachernode, below of=teacher2] {pool};
\node (fc) [teachernode, below of=pool]{fc};
\node (student00) [studentnode, right of=teacher0, yshift=-0.5cm] {\(s_{00}\)};
\node (student01) [studentnode, right of=student00] {\(s_{01}\)};
\node (dots0n) [dotsnode, right of=student01] {\(\cdots\)};
\node (student0n) [studentnode, right of=dots0n] {\(s_{0n}\)};
\node (student10) [studentnode, right of=teacher1, yshift=-0.5cm] {\(s_{10}\)};
\node (student11) [studentnode, right of=student10] {\(s_{11}\)};
\node (dots1n) [dotsnode, right of=student11] {\(\cdots\)};
\node (student1n) [studentnode, right of=dots1n] {\(s_{1n}\)};
\node (student20) [studentnode, right of=teacher2, yshift=-0.5cm] {\(s_{20}\)};
\node (student21) [studentnode, right of=student20] {\(s_{21}\)};
\node (dots2n) [dotsnode, right of=student21] {\(\cdots\)};
\node (student2n) [studentnode, right of=dots2n] {\(s_{2n}\)};
\draw [infarrow] (stem) -- (student01);
\draw [infarrow] (student01) -- (student10);
\draw [infarrow] (student10) -- (teacher2);
\draw [infarrow] (teacher2) -- (pool);
\draw [infarrow] (pool) -- (fc);

\end{tikzpicture}
\caption{Search}
\end{subfigure}
\end{figure}
